Ver: View Discovery in the Wild

We present Ver, a data discovery system that identifies project-join views over large repositories of tables that do not contain join path information, and even when input queries are inaccurate. Ver implements a reference architecture to solve both the technical (scale and search) and human (semantic ambiguity, navigating a large number of results) problems of view discovery. We demonstrate users find the view they want when using Ver with a user study and we demonstrate its performance with large-scale end-to-end experiments on real-world datasets containing tens of millions of join paths.

==> sections/4c_backup.tex <==
\section{View Distillation}
\label{sec:vdistillation}

%\zz{I have modified this section based on the comments}

\update{}{\textsc{View-Distillation} analyzes the views produced by the \textsc{join-graph-search} and computes \emph{relationships}, including the novel \emph{4C}, that are used to reduce the number of views and as part of \textsc{view-presentation}.}

%Specifically, it outputs a graph where each view is a node and a related collection of view pairs are labelled with the identified relationships. }


% The goal of the \textsc{view distillation} component is to collect and generate \emph{signals} that helps to automatically prune out certain candidate PJ-views and help \textsc{view-presentation} efficiently choose the right candidate view for an interface. Collected signals include column headers, source of constituent tables, join paths, and their similarity with input examples. These signals are computed by building an inverted index over the tokens present in the repository along with the join path index generated by the discovery index component. In addition, the \textsc{signal-generation} component generates a class of novel signals, called \textit{4C}, that help reduce the size of the candidate PJ-views.

\mypar{4C Signals} Output views with the same schema are classified into \update{}{the following} categories:

\begin{definition}[Compatible views]
Two candidate views, $V_1$ and $V_2$, are compatible if they have the same set of tuples $(V_1 \cap V_2) =  V_1=V_2$.
\end{definition}

\begin{definition}[Contained views]
A view, $V_1$, contains another view, $V_2$, when $V_2\subseteq V_1$, that is, when all rows of $V_2$ are contained in $V_1$.
\end{definition}

% \mypar{4C Signals} Output views with the same schema are classified into four categories: \textit{Compatible}, which means that views are identical; \textit{Contained}, which means that the values of one view subsume others; \textit{Complementary}, which means that the set difference of tuples of views is not empty; and \textit{Contradictory}, which means that tuples from different tables with same key disagree on at least one of their attributes' values. Depending on the chosen key, two views may be \emph{complementary} or \emph{contradictory}. We consider all columns that uniquely define rows as candidate keys for a view. To define these signals, we refer to a view $V_i$ as a set of tuples in the dataset with $k(V_i)$ denoting the set of values corresponding to its candidate key.

Views can also be \emph{Complementary} and \emph{Contradictory}, and this depends on their candidate key.
\sg{Change to view pair?}
\begin{definition}[Candidate key]
A candidate key, $\mathcal{K}$, is a set of attributes in an output view, $V_i$, that can uniquely identify each row in $R_i$. We can refer to a row, $r_i \in R_i$, with its candidate key value, $\mathcal{K}_i$, which we can use to obtain the row; $\mathcal{K}(R_i, \mathcal{K}_i) = r_i$. There can be multiple candidate keys in $V_i$ that satisfy this property. 
\end{definition}

\begin{definition}[Complementary views]
Two views, $V_1$ and $V_2$ are complementary if the two views have the same candidate key, $\mathcal{K}$, and $|(K_1 \setminus K_2)| > 0$ and $|(K_2 \setminus K_1)| > 0$, where $K_1$ and $K_2$ are the set of candidate key values for $V_1$ and $V_2$ respectively. That is, each view has candidate key values not contained in the other view.
\end{definition}

\begin{definition}[Contradictory views]
Two views, $V_1$ and $V_2$ are contradictory if the two views have the same candidate key, $\mathcal{K}$, and a key value that exists in both views, $\mathcal{K}_i \in K_1, K_2$, yields distinct rows, $\mathcal{K}(V_1; \mathcal{K}_i) \neq \mathcal{K}(V_2; \mathcal{K}_i)$. Two rows are distinct when any value of any of their attributes is different. 

\end{definition}
\update{}{Algorithm}~\ref{alg:4c_main} \update{}{presents \texttt{\textbf{Ver}}'s approach to identify 4C signals. First, it initializes the graph $G$ where each view is added as a node, identifies keys in each view (line 1) and  partitions the collection of views $\mathbbm{V}$ into different groups $\mathcal{V}$ based on their schema (line 2). All views with same schema are present in the same partition and will be compared for subsequent processing. These schema-based groups are processed sequentially to identify relationships (line 3). The relationship identification process operates in two phases. The first phase (lines 4-13) hashs all views (hash value of view $V$ is denoted by $H(V)$) and compares hashed values to check containment and compatibility.  A pair of views $V_i$ and $V_j$ that overlap but are not contained or compatible are marked as complementary. These pairs are later updated to be contradictory if the second phase identifies any contradictions. Note that the hashing process maps each view to a set of values, where each value corresponds to row in the original view and we employ a cache to not hash any view multiple times.  The second phase constructs an inverted index over the values in the key column(s) of each view in the partition $\mathcal{V}$. This index maps each key value (say $k$) to a list of rows that contain the value $k$ (denoted by $I[k]$).
\texttt{\textbf{Ver}} iterates over all values of the key column and identifies contradictions among the rows that contain the value (line 16-18). Specifically, it groups all duplicate rows that contain a key $k$ together (line 16) and any pair of views that are not in the same group are contradictory (line 17-18).  }


%\update{}{Note that although the description above refers to two views, the 4C method classifies multiple views into each of the above categories. For example, a view can be compatible with other views, contains other views, and be complementary or contradictory to other views on a candidate key, all at the same time.
%Next, we present the algorithm we use to classify the output views into the four above categories.}
\sg{use category not relationship/signal}
{
\IncMargin{1em}
\begin{algorithm}\SetKwFunction{Union}{Union}
\scriptsize
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{$\mathbbm{V}$, collection of views}
\Output{ $G$, views classified per category and schema type}
 \BlankLine
 $G\leftarrow \textsc{Add-Nodes}(\mathbbm{V})$,$\mathbbm{V}\leftarrow \textsc{Identify-Keys}(\mathbbm{V})$\\
 $\mathbbm{V} \leftarrow \textsc{Schema-based-partition}(V)$\\
 \For{$\mathcal{V} \in \mathbbm{V}$}{
 \For{$1\leq i,j\leq |\mathcal{V}|, i>j$}{
    $V_i\leftarrow \mathcal{V}[i], V_j\leftarrow \mathcal{V}[j]$\\
    \tcc*[h]{\scriptsize Iterate over the views, compare rowwise hashes $H$}\\
    \If{$H[V_i] = H[V_j]$ }{
        $G[(V_i,V_j)]=$ Compatible\\
        $\mathcal{V}\leftarrow \mathcal{V}\setminus\{V_i\}$\\
        }
    \ElseIf{$H[V_i] \subset H[V_j]$ \text{ or } $H[V_j] \subset H[V_i]$   }{
    {   
        $G[(V_i,V_j)]=$ Contained\\
        $\mathcal{V}\leftarrow \mathcal{V}\setminus\{V_i,V_j\} \cup \{V_i\cup V_j\}$\\
    }}
    \ElseIf{$H[V_i] \cap H[V_j]\neq \phi$ }{
    {
    \tcc*[h]{\scriptsize Initialize any overlapping view pair as complementary}\\ 
        $G[(V_i,V_j)]=$ Complementary\\
    }
    }
    
 }
 \tcc*[h]{\scriptsize Second phase: Identify contradictions}\\
 $I\leftarrow \textsc{Inverted-Index}(\mathcal{V})$\\
  \For{$k\in I.\texttt{keys}()$}{
    $\mathcal{C} \leftarrow \textsc{Group} (I[k])$\\
    \tcc*[h]{\scriptsize Identify pairs in different groups}\\
    \For{$(V_i,V_j) : V_i,V_j\in I[k],~ \mathcal{C}[V_i] \neq \mathcal{C}[V_j]$}{
    $G[(V_i,V_j)]=$ Contradictory
    }
  }
 }
 \caption{\update{}{View Distillation}}
 \label{alg:4c_main}
\end{algorithm}
}
\begin{algorithm}
\scriptsize
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$V$, collection of output views}
\KwOutput{$G$, views classified per class and schema type}
 \BlankLine
 $S \leftarrow classify\_per\_schema(V)$\; \label{4c_main:classify_per_schema}
 \For{$s \in S$}{ \label{4c_main:loop_schema}
    $C1 \leftarrow identify\_c1(V)$\; \label{4c_main:c1}
    $SC1 \leftarrow select\_representative\_c1(C1)$\; \label{4c_main:select_representative_c1}
    $C2, C34 \leftarrow identify\_c2\_and\_candidate\_c3c4(SC1)$\; \label{4c_main:c2} 
    $C3, C4 \leftarrow identify\_c3\_and\_c4(candidate\_C3C4)$\; \label{4c_main:c3_c4} 
    $G[s] \leftarrow (C1, C2, C3, C4)$\;
 }
 \Return $G$\;
 \caption{\update{}{Main 4C}}
 \label{4c_main}
\end{algorithm}

\update{}{The main body of the algorithm is shown in Algorithm} \ref{4c_main}\update{}{. Because 4C works on views with the same schema (attributes in this case), the first step is to separate the output views into groups according to their schema (line }\ref{4c_main:classify_per_schema}\update{}{). Then, the algorithm runs the 4C classification for each schema group (line }\ref{4c_main:loop_schema}\update{}{), leading to the classification of views into the four categories: \textit{compatible} ($C1$), \textit{contained} ($C2$), \textit{complementary} ($C3$), and \textit{contradictory} ($C4$). It will first identify quickly the compatible and contained views. Then, it identifies complementary and contradictory views among the remaining ones.}

\begin{algorithm}
\scriptsize
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$V$, collection of output views}
\KwOutput{$C1$, collection of lists, each list contains $v \in V$ that are compatible. $hashes$, map from view to its hashes}
 \BlankLine
 $g \leftarrow map()$\;
 $hashes \leftarrow map()$\;
 \For{$v_i \in V$}{
    $hv_i \leftarrow hash(v_i)$\; \label{4c_compatible:hash}
    $add(g, hv_i.sum(), v_i)$\; \label{4c_compatible:add}
    $add(set(hashes), v_i, hv_i)$\; \label{4c_compatible:save}
 }
 $C1 \leftarrow g.values()$\;
 \Return $(C1, hashes)$\;
 \caption{\update{}{identify\_c1}}
 \label{4c_compatible}
\end{algorithm}

\mypar{\update{}{Identify compatible views}}\update{}{ The next step is to identify groups of views that are compatible ($C1$) with each other, as shown in Algorithm} \ref{4c_compatible}\update{}{. The main idea is to hash each view (line }\ref{4c_compatible:hash}\update{}{), and insert the view on a map that is keyed on the hash value (line }\ref{4c_compatible:add}\update{}{). A view hash is the sum of its rows hashes, and a row hash is the sum of its cells hashes. With this hashing method, compatible views are guaranteed to have the same hash value, so this is an efficient way of identifying groups of compatible views fast. Additionally, the set of row hashes of each view is saved in another map and returned (line }\ref{4c_compatible:save}\update{}{, so we don't have to recompute the hashes in later step.}

\update{}{Because all compatible views are identical, in the Main 4C algorithm, we select one only to continue the classification (line }\ref{4c_main:select_representative_c1}\update{}{). The selected views are then given to a function in charge of identifying contained groups ($C2$), as well as groups that may be either complementary or contradictory ($C34$), see Algorithm }\ref{4c_main:c2}.

\begin{algorithm}
\scriptsize
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$SC1$, collection of output views. $hashes$, map from view to its hashes}
\KwOutput{$C2$, list of views $v \in V$, each view is the largest view in its contained group \zz{?}. $C34$, list of views $v \in V$ that are either contradictory or complementary
% $C2$, list of tuples $(v_C, [vc])$; $v_C$ contains all $[v_c]$. $C34$, list of tuples $(v_i, v_j, I_i, I_j )$; $I_{i,j}$ are the sets of row indices in which $v_i$ and $v_j$ disagree
}
 \BlankLine
%  $(gc2, gc34) \leftarrow (map(), map())$\;
$C3, C34 \leftarrow set(), set()$\;
 $pruned \leftarrow set()\leftarrow$ contained views to be pruned\\
%  \For{$(v_i, v_j) \in pair(SC1)$}{ \label{4c_contained:loop}
\For{$v_i \in SC1$}{
    \uIf{$v_i \in pruned$}{
            $continue$\;
        }
    \For{$v_j \in SC1$}{
        % $(h\_list_i, h\_list_j) \leftarrow (hash\_rows(v_i), hash\_rows(v_j))$\;
        \uIf{$v_j \in pruned$}{
            $continue$\;
        }
        $l\_v \leftarrow None$ $\leftarrow$ largest contained view in this iteration\\ \label{4c_contained:initialize_largest}
        $(h\_set_i, h\_set_j) \leftarrow (hashes.get(v_i), hashes.get(v_j))$\; \label{4c_contained:get_hash}
        % $(h\_set_i, h\_set_j) \leftarrow (set(hv_i), set(hv_j))$\; \label{4c_contained:get_hash_end}
        \uIf{$h\_set_i.is\_subset(h\_set_j)$}{         \label{4c_contained:if_start}
            \uIf{$l\_v$ == None}{
                $l\_v \leftarrow v_j$\;
            }
            \uElseIf{$v_j.size() > l\_v.size()$}{
                $add(pruned, l\_v)$\;
                $l\_v \leftarrow v_j$\;
            }
            $add(pruned, v_i)$\; \label{4c_contained:if_end}
        }
        \uElseIf{$h\_set_j.is\_subset(h\_set_i)$}{ \label{4c_contained:mirror}
            \tcc*[h]{Mirror of the above}\\ 
        }
        % \eIf{$len(h\_set_i) \geq len(h \_set_j)$}
        % { \label{4c_contained:if_start}
        %     \If{$(h\_set_j \setminus h\_set_i) = 0$}{
        %         $add(gc2, v_i, v_j)$\;
        %     }
        % \label{4c_contained:if_end} }
        % { \label{4c_contained:else_start}
        %     $s_{ij} \leftarrow h\_set_i \setminus h\_set_j$\;
        %     $s_{ji} \leftarrow h\_set_j \setminus h\_set_i$\;
        %     \If{$s_{ij} \geq 0 \land s_{ji} \geq 0$}{
        %         $I_i \leftarrow indices(h\_list_i, s_{ij})$\;
        %         $I_j \leftarrow indices(h\_list_j, s_{ji})$\;
        %         $add(gc34, v_i, v_j, I_i, I_j)$\;
        %     }
        % } \label{4c_contained:else_end}
    }
    \uIf{$l\_v$ != $None$}{
        $add(C3, l\_v)$\;
    }
 }
 $C34 \leftarrow SC1 \setminus pruned$\; \label{4c_contained:c34}
%  $(C2, C34) \leftarrow (unpack(gc2), unpack(gc34))$\;
 \Return $(C2, C34)$\;
 \caption{\update{}{identify\_c2\_and\_candidate\_c3c4}}
 \label{4c_contained}
\end{algorithm}

\mypar{\update{}{Identify contained views}} \update{}{The function to finding contained views is shown in Algorithm }\ref{4c_contained}\update{}{. For each pair of views, the algorithm obtains the set of row hashes of each view (line }\ref{4c_contained:get_hash}\update{}{. The largest contained view, $l\_v$, for the current contained group is initialized (line }\ref{4c_contained:initialize_largest}\update{}{. Lines }\ref{4c_contained:if_start}--\ref{4c_contained:if_end}\update{}{ checks whether the row hashes of one view, $v_i$, are completely contained in another view, $v_j$, in which case the $v_i$ is contained in $v_j$. The largest contained view is assigned by comparing its current size and $v_j$'s size. The smaller contained views are pruned and will not be compared in later iterations. Finally, all views except the pruned views are assigned as candidate complementary and contradictory views (line }\ref{4c_contained:c34}\update{}{). 
% The algorithm returns the largest view of each identified groups of contained views as well as views that may be complementary or contradictory.
} 
% For each pair of views (line }\ref{4c_contained:loop}\update{}{), the algorithm obtains the list and the set of hashes of each view respectively. The list will be used to identify indexes of rows (because it maintains the order), while the sets are used to quickly tell whether the views are contained or may be complementary. Lines }\ref{4c_contained:if_start}--\ref{4c_contained:if_end}\update{}{ checks whether the hashes of one view are completely contained on the first, in which case the view is contained in the first and this is recorded in the variable $gc2$. Note that because the loop enumerates pairs of views in both directions, it is not necessary to check for containment in both directions here.}

% \update{}{If the views are not contained, the algorithm tries to decide if they are candidates for the complementary and contradictory group. This decision is done in lines }\ref{4c_contained:else_start}--\ref{4c_contained:else_end}\update{}{. The algorithm computes the set difference of rows in both directions and checks whether it is non-empty in both cases. When it is, this indicates that each view has hashes not contained in the other view. This can be caused for two different reasons: either one view has rows that are non existent in the other (a case of complementarity), or the values of certain rows differ in some values, which would also lead to different hashes and indicate a contradiction. The algorithm returns the identified groups of contained views as well as those that may be complementary or contradictory.}

\begin{algorithm}
\scriptsize
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$C34$, list of candidate complementary and contradictory views
% list of tuples $(v_i, v_j, I_i, I_j)$; $I_{i,j}$ are the sets of row indices in which $v_i$ and $v_j$ disagree
}
\KwOutput{$C3$, list of tuples $(v_i, v_j, \mathcal{K})$, where $v_i$ and $v_j$ are complementary on candidate key $\mathcal{K}$. $C4$, list of tuples $(v_i, v_j, \mathcal{K}, K)$, $K$ is the set of key values of candidate key $\mathcal{K}$ in which $v_i$ presents a contradiction with respect to $v_j$
% $C3$, list of tuples $(v_i, v_j, k, K_i, K_j)$, $K_{i,j}$ are the sets of key values of candidate key $k$ in $v_i$ and $v_j$ that are complementary. $C4$, list of tuples $(v_i, v_j, k, K)$, $K$ is the set of key values of candidate key $k$ in which $v_i$ presents a contradiction with respect to $v_j$
}
 \BlankLine
 $(C3;C4) \leftarrow (set(), set())$\;
 \tcc*[h]{Builds an inverted index for each candidate key and key value. $I[\mathcal{K}][\mathcal{K}_i] = V_i$, where $V_i$ are the list of views with candidate key $\mathcal{K}$ and key value $\mathcal{K}_i$}\\ 
 $I = build\_inverted\_index(C34)$\; 
 %\For{$V_i \in I_k \forall I_k\in I$}
 \For{$(\mathcal{K}, I_\mathcal{K}) \in I$}{
    \For{$(\mathcal{K}_i, V_i) \in I_k$}{
        \tcc*[h]{Views with the same row belong to the same cluster}\\ 
        $clusters = map()$\;
        \For{$v \in V_i$}{
            $r = \mathcal{K}(R_i, \mathcal{K}_i) \leftarrow$ get row from key value\\
            $add(clusters, r, v)$\;
        }
        \tcc*[h]{Views in each cluster is contradictory to views in all other clusters}\\ 
        \For{$(r, v\_list) \in clusters$}{
            \For{$v_i \in v\_list$}{
                $v\_other = clusters.values() \setminus v\_list$\;
                \For{$v_j \in v\_other$}{
                    $add(C4, v_i, v_j, \mathcal{K}, \mathcal{K}_i)$\;
                }
            }
        }
    }
 }
 \For{$(v_i, v_j, \mathcal{K}) \in get\_tuple(C4)$}{
    \uIf{! $v_i[K].is\_disjoint(v_i[K])$}{
        \tcc*[h]{$v_i$ and $v_j$ are complementary if they have overlapping key values}\\ 
        $add(C3, v_i, v_j, \mathcal{K})$\;
    }
 }
%  \For{$(v_i, v_j, I_i, I_j) \in C34$}{ \label{4c_contra_compl:loop}
%     $vsel_i \leftarrow select(v_i, I_i)$\; \label{4c_contra_compl:select_i}
%     $vsel_j \leftarrow select(v_j, I_j)$\; \label{4c_contra_compl:select_j}
%     $k\_list \leftarrow find\_candidate\_keys(v_i, v_j)$\; \label{4c_contra_compl:find_keys}
%     \For{$k \in k\_list$}{ \label{4c_contra_compl:for_key}
%         $KV_i \leftarrow project(vsel_i, k)$\; \label{4c_contra_compl:project_i}
%         $KV_j \leftarrow project(vsel_j, k)$\; \label{4c_contra_compl:project_j}
%         $K\_intersect \leftarrow KV_i \cap KV_j$\; \label{4c_contra_compl:k_intersect}
%         $K \leftarrow find\_contr(vsel_i, vsel_j, K\_intersect)$\; \label{4c_contra_compl:find_contr}
%         $add(C4, v_i, v_j, k, K)$\;
%         \If{$len(K) = 0$}{
%             $K\_compl \leftarrow (KV_i \cup KV_j ) \setminus K\_intersect$\;  \label{4c_contra_compl:k_compl}
%             $(K_i, K_j) \leftarrow find\_compl(vsel_i, vsel_j, K\_compl)$\; \label{4c_contra_compl:find_compl}
%             $add(C3, v_i, v_j, k, K_i, K_j)$\;
%         }
%     }
%  }
 \Return $(C3, C4)$\;
 \caption{\update{}{identify\_c3\_and\_c4}}
 \label{4c_contra_compl}
\end{algorithm}

\mypar{\update{}{Identify complementary and contradictory views}} \update{}{The last part of the algorithm is to identify which pairs of views in C34 are complementary and which are contradictory.} \zz{checkpoint}
% This corresponds to line }\ref{4c_main:c3_c4}\update{}{ in the main body of Algorithm }\ref{4c_main}\update{}{. The body of this function is shown in more detail in Algorithm }\ref{4c_contra_compl}\update{}{. For each pair of views (line }\ref{4c_contra_compl:loop})\update{}{, it checks whether the different values (hashes) identified between this pair are due to complementarity or contradictions. For that, it first selects the relevant rows from each view (lines }\ref{4c_contra_compl:select_i}--\ref{4c_contra_compl:select_j})\update{}{ and obtains all possible candidate keys, $k\_list$ of the two views (line }\ref{4c_contra_compl:find_keys}\update{}{). Then for each candidate key (line }\ref{4c_contra_compl:for_key}\update{}{), it projects the attributes of that key into the selection (lines }\ref{4c_contra_compl:project_i}--\ref{4c_contra_compl:project_j}\update{}{). This
% produces $KV_i$ and $KV_j$ , which are the sets of key values that correspond to the distinct hashes of each view. At this point, the intersection of these two sets, $K\_intersect$, corresponds to the contradictory examples (lines }\ref{4c_contra_compl:k_intersect}--\ref{4c_contra_compl:find_contr}\update{}{), while the rest of values, $K\_compl$, correspond to the complementary ones (lines }\ref{4c_contra_compl:k_compl}--\ref{4c_contra_compl:find_compl}\update{}{). Two views are only complementary if no contradictions exist. Therefore, each candidate key of a pair of views corresponds either contradictory or complementary relationship.


% \smallskip
% Once finished, all views will be classified into the four categories. By applying the \textit{4C} method, we are able to prune a portion of the output views; e.g. we can discard \textit{compatible} views, leaving only one view in each group, and choose the view with the highest cardinality among each group of \textit{contained} views \zz{since ... (need reasons)}. The user still has to choose among the rest of the views. The most naive approach would be letting the user look through all the rest of views and choose their preferred one, but this approach can be very ineffective and tedious for the user since the amount of views left may still be very large and and views can be noisy and spurious. To leverage the \textit{complementary} or \textit{contradictory} relationships we obtained using the \textit{4C} method, we designed a \textit{human-in-the-loop} presentation framework that reduces user's effort and guide them towards their preferred view with minimal amount of interactions by asking them questions strategically.


% \mypar{Efficiently computing 4C signals} The algorithm iteratively partitions pairs of candidate views into the 4 categories. To avoid cell-level comparison of values and efficient comparison of views, we construct a hash for each row. Compatible and contained views are classified first by comparing row hashes, the rest of views are classified to either complementary views or contradictory views based on the candidate keys and their associating values. 

% It hashes view rows for more efficient comparison.

% Using this formalism, our \textit{4C} classification algorithm iteratively partitions pairs of candidate views into the four categories. To avoid cell-level comparison of values and efficient comparison of views, we construct a hash for each row.


\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$M$, double-nested map where the first key is the view pair $(v_i, v_j)$ that exist in $C4$, and the second key is its candidate key $\mathcal{K}$, with the corresponding value $K$, the set of key values of candidate key $\mathcal{K}$ in which $v_i$ presents a contradiction with respect to $v_j$. $sample\_size$, maximum number of contradictory or complementary rows in a signal}
\KwOutput{$S\_contra$, lists of contradictory signals consisting of tuple $(\mathcal{K}, S_1, S_2, R_1, R_2)$.}
 \BlankLine
 \ForEach{$(v_i, v_j) \in M$}{
    \ForEach{$\mathcal{K} \in M[(v_i, v_j)]$}{
        $(S_1,  S_2) \leftarrow (set(), set())$\;
        $(R_1,  R_2) \leftarrow (set(), set())$\;
        $K \leftarrow M[(v_i, v_j)][\mathcal{K}]$\;
        $SK \leftarrow sample(K, sample\_size)$\; \label{generate_signals:sample_contra}
        \For{$\mathcal{K}_i \in SK$}{
            $r_1 \leftarrow \mathcal{K}(R_i, \mathcal{K}_i)$\;
            $r_2 \leftarrow \mathcal{K}(R_j, \mathcal{K}_i)$\;
            $(s_1, s_2) \leftarrow get\_contra\_set(r_1, r_2)$\; \label{generate_signals:get_contr_set}
            $add(S_1, s_1)$\; \label{generate_signals:combine_contra_start}
            $add(S_2, s_2)$\;
            $add(R_1, r_1)$\;
            $add(R_2, r_2)$\;\label{generate_signals:combine_contra_end}
        }
        $add(S\_contra, k, S_1, S_2, R_1, R_2)$\;
    }
 }
 \Return $S\_contra$\;
 \caption{\update{}{generate\_contradictory\_signals}}
 \label{generate_signals}
\end{algorithm}

\update{}{Once finished, all views will be classified into the four categories. Then, for each pair of view, we can generate }\textit{\update{}{contradictory signals}}\update{}{ as shown in Algorithm }\ref{generate_signals}\update{}{. First, we introduce the definition of a }\textit{\update{}{contradictory set}}. \zz{I want to remove the part about contradictory signals since this strategy is only used in one experiment in evaluation, to prune more views in each interaction}

\begin{definition}[\update{}{Contradictory set}]
\update{}{Two sets of views, $s_1 \subseteq V$ and $s_2 \subseteq V$, form a \textit{contradictory set}, if they all share the same candidate key, $\mathcal{K}$, and there exists a key value, $k$, such that for all the views $v_i \in s_1$, the row $r_1 = k(R_i; k)$ is the same; for all the views $v_j \in s_2$, the row $r_2 = k(R_j; k)$ is the same. Finally, $r_1 \neq r_2$, meaning $r_1$ and $r_2$ is contradictory on the key value $k$, which is present in all the views in both $s_1$ and $s_2$.}
\end{definition}

A \emph{contradictory signal} consists of the rows with contradictory values, and their corresponding \emph{contradictory sets} of PJ-views containing those contradictory values. For example, suppose the candidate PJ-views have the attributes \textit{name} and \textit{address}, where \textit{name} is a valid candidate key. A contradictory signal may contain two contradictory rows corresponding to the candidate key value \textit{Alice}; one row has Alice's work address, while the other has Alice's home address. Then, all candidate PJ-views that share the same candidate key, \textit{name}, will be grouped into two contradictory sets -- the set of PJ-views that contain the row with Alice's work address, and the set of PJ-views that contain the row with Alice's home address.


We construct contradictory signals by leveraging the \emph{transitive} relationship of contradictory rows among views\update{}{, as shown in Algorithm }\ref{generate_signals}\update{}{. Depending on the candidate key of each pair of view, we sample certain number of contradictory rows (line }\ref{generate_signals:sample_contra}\update{}{), and obtain the corresponding contradictory set for each sampled row (line }\ref{generate_signals:get_contr_set} \zz{there are more stuff happening for how to get the contradictory set but I am omitting the details here}\update{}{). We then combine them together so that each signal contains multiple rows along with the combined contradictory set (lines }\ref{generate_signals:combine_contra_start}--\ref{generate_signals:combine_contra_end}. The sampling approach allows more PJ-views to be grouped into the contradictory set, thus reducing the view search space.

% For each pair of \emph{contradictory signals}, we generate a signal that contains the rows with contradictory values and their respective \emph{contradictory sets}. 

% Since the contradictory views are inherently discriminative, we construct \textit{contradictory signals} from the contradictory views by leveraging the \textit{transitive} relationships of contradictory rows among those views. For each pair of contradictory views, we generate \textit{contradictory signals} consisting of rows with contradictory values and their respective \textit{contradictory sets}. For example, suppose the candidate PJ-views have the attributes \textit{name} and \textit{address}, where \textit{name} is a valid candidate key. A contradictory signal may contain two contradictory rows corresponding to one candidate key value \textit{Alice}, one has Alice's work address, while the other has Alice's home address. Then, all candidate PJ-views that share the same candidate key, \textit{name}, will be grouped into two contradictory sets consisting of PJ-views that contain the row with Alice's work address and Alice's home address respectively. A contradictory signal includes one or multiple contradictory rows, which are sampled from pairs of contradictory views. Using this approach, each contradictory signal can involve many views on each side, thus further reduce the view choice space.


\mypar{Using 4C signals to reduce candidate PJ-view space}
\label{subsec:chosenstrategy}
% We discuss how 4C signals help to reduce the number of the candidate PJ-views.
% The 4C signals can be sent downstream to the \textsc{view- presentation} stage to help users select an adequate PJ-view, or used within the signal generation component to reduce the size of the candidate PJ-view space. We explain how to leverage them for the latter goal. 
Compatible views are summarized into a single view. Contained views are represented by the largest cardinality view. Complementary views are unioned. These first three actions are carried downstream with \emph{provenance} of the operation to permit downstream users reverse them when they are wrong, \eg unioning ``2016'' data with ``2017'' may not always be appropriate for the downstream goal. Contradictory views cannot be processed automatically. They arise due to: i) view was produced using a wrong join path; ii) the original data is contradictory, \eg due to semantic ambiguity. Contradictory signals are forwarded to the \textsc{view-presentation} component when their discriminatory power is high, \ie when the expected number of views pruned after a user selection is high.

% Compatible views are summarized into a single view. When there is a group of contained views, the view with the largest cardinality pervades. When views are complementary, they are unioned. Finally, it is not possible to make an automated decision for contradictory views. Contradictory views usually arise for two reasons: i) view was produced using a wrong join path; ii) the original data is contradictory, \ie due to semantic ambiguity. A user may be able to tell apart the right view, thus selecting a join path \emph{a posteriori}. Without a user, we cannot automatically decide on which contradictory value in each contradictory signal is correct, but it is possible to determine whether the signal is useful or not, based on its information gain and consequently decide whether to query the user or not---with the intention of avoiding sending non-discriminatory and hence useless signals. Contradictory signals are sorted according to their degree of discrimination, which is defined as the expected number of views in a contradictory set it would prune after a selection of its respective contradictory rows is made. 
% We will show the effectiveness of this approach in the evaluation section.


==> sections/architecture.tex <==
\section{A Reference Architecture}
\label{sec:architecture}

% In this section, we present a reference architecture.

\myparwod{Why a Reference Architecture?} From a systems engineering perspective, a reference architecture is the materialization of a ``divide and conquer'' strategy that splits complex engineering problems into smaller parts. Thus, a reference architecture describes a collection of components and their interactions. In making a reference architecture concrete, we state our understanding of the problem and represent it as a concrete artifact that the community can scrutinize and improve.

\subsection*{Design Overview}

Finding a PJ-view in the wild requires solving a \emph{human} and a \emph{technical} problem. We present a reference architecture for view discovery that contains components targeting both \emph{human} and \emph{technical} problems. Along with each component, we discuss implementation options, including those made by \sys{}. We also briefly discuss two novel components, \textsc{View Distillation} and \textsc{View Presentation}.


% along with  with \sys{}'s implementation that contains components targeting both problems.

% , and focus on the implementation of an engine called \textbf{\sys{}}. 

\mypar{Overview} Algorithm~\ref{algo_dod} shows pseudocode (human components are {\color{Blue}highlighted in blue}) and \F\ref{fig:architecture} shows \sys{}'s architecture inside a funnel, denoting the gradual reduction of views as data flows downstream. \sys{} builds a discovery index offline. 

% (see top of \F\ref{fig:architecture}).

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize Discovery Engine and Index Creation (technical)}}]
      
% \vspace{-1ex}

\mypar{\textsc{Discovery Engine and Index Creation (technical)}} \emph{This component builds indices over pathless table collections: i) a join path index, which can be approximate; ii) retrieval indices over table names, values, attribute names and column similarity. The indices are available online, via the Engine's API to other components. (\textbf{Challenge 2}).}

% \vspace{0ex}
% \end{tcolorbox}

% This path information is made available online to the other components. In addition to this index, the PPE problem requires 
% Users provide input examples $\chi$, via a \textsc{view-specification} component to design and submit queries, which may contain noisy values (Challenge 1). 

The indices can be built using state-of-the-art methods such as Aurum~\cite{aurum} (that \sys{}'s implementation uses), Auctus~\cite{auctus}, JOSIE~\cite{zhu2019josie}, LSHEnsemble~\cite{zhu2016lsh}. After the indices are built, users design and submit queries via a \textsc{view-specification} component (line 1).
% , where they provide examples, $\chi$.

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize View Specification (human)}}]
      
% \vspace{-0ex}

\mypar{\textsc{View Specification (human)}}
Discovery interfaces include spreadsheet-style, keyword search, APIs, natural language, and combinations of these. The reference architecture supports these interfaces via the \textsc{View-Specification} component. For QBE-based interfaces, as implemented by \sys{}, the input is a set of examples, $\chi$, and the output of this stage is a set of example attributes and values. \textsc{View-Specification} may interact with users when it detects the provided examples are ambiguous, or to offer examples to choose from.

% \vspace{0ex}
% \end{tcolorbox}

Next, the \textsc{column-selection} component selects the subset of tables containing user-provided examples, $\chi$ (lines~\ref{dodline3}-\ref{dodline7}).

% The QBE-style examples and index are then considered by the \textsc{column-selection} component to shortlist a subset of the pathless table collection that contains input example values (lines~\ref{dodline3}-\ref{dodline7}). This component can run with or without human guidance. When guidance is available, it helps to narrow down the candidate columns and tables relevant for the desired view. \textsc{Column-selection} outputs a collection of tables and respective columns that contain input examples (\textsc{Cand}). 

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize Column Selection (technical)}}]
      
% \vspace{-0ex}

\mypar{\textsc{Column Selection (technical)}} \emph{This component must be designed to identify relevant data even when the input query is noisy, addressing \textbf{Challenge 1} above. The output of this component is a collection of candidate tables and columns.}

% \vspace{0ex}
% \end{tcolorbox}


\begin{algorithm}[t]
    \scriptsize
    \SetKwFunction{Union}{Union} \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	
	\Input{Pathless table collection $\D$, Discovery Index $I$} 
	\Output{PJ-views $\mathcal{V}$}
	 \BlankLine 
	 \bluecolor{$\chi \leftarrow\textsc{View-Specification}(\mathcal{D})$}\\
	 $\textsc{Cand}\leftarrow \phi$\\%\\\tcc*[f]{Initialize candidate columns}\\
	 \For{$\chi.A_i\in \textsc{Columns}(\chi)$\label{dodline3}}{ %\tcc*[f]{Iterate over columns in input query}\\
	    $\textsc{Cand}(A_i) \leftarrow \textsc{Column-Selection} (\chi.A_i, \D, I)$\\%\tcc*[f]{Identify matching columns}\\
	    \If{\textsc{Mode}==Interactive}{
	   \bluecolor{ $\textsc{Cand}(A_i)\leftarrow $ Query $\textsc{Cand}(A_i)$} \\
	    }
	    $\textsc{Cand}\leftarrow	    \textsc{Cand}\cup \textsc{Cand}(A_i)$\label{dodline7}
	}
	$\mathcal{V}_{PJ} \leftarrow \textsc{Join-Graph-Search} (\textsc{Cand},\chi)$\label{dodline8}\\
	$\mathcal{S} \leftarrow \textsc{View-Distillation} (\mathcal{V}_{PJ})$\label{dodline9}\\
	\If{\textsc{Mode}==Interactive\label{dodline10}}{
	\bluecolor{$\mathcal{V} \leftarrow \textsc{View-Presentation}(\mathcal{V}_{PJ},\mathcal{S})$} 
	}
	\Else{
	$\mathcal{V} \leftarrow $ Rank $\mathcal{V}_{PJ}$ based on overlap score\label{dodline13}
	}
	 \Return $\mathcal{V}$
 	 	  \caption{\sys{} Design Overview %\notera{can we mark in blue or green the lines that refer to human components?}
 	 	  }
 	 	  \label{algo_dod} 
\end{algorithm}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/architecture.pdf}
  %\includegraphics[width=\linewidth]{figures/Architecture_digital.pdf}
  \caption{\sys{} Reference Architecture. The funnel illustrates the progressive reduction of data as it flows downstream.}
  \label{fig:architecture}
\end{figure}

The candidate columns are processed by the \textsc{join-graph-search} component (line~\ref{dodline8}) to enumerate and materialize candidate PJ-views (addresses Challenge 3). The candidate view search space reduces, as shown in \F\ref{fig:architecture}.

% Due to the noise of datasets and input query, the \textsc{join-graph-search} component may generate many candidate PJ-views ({Challenge 4}). 

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize Join Graph Search (technical)}}]
      
% \vspace{-0ex}

\mypar{\textsc{Join Graph Search (technical)}} \emph{Given a set of candidate tables, an input query, and the discovery index providing join paths, this component identifies all \emph{join graphs} that, when materialized, produce candidate PJ-views. The main goal of this component is to address the large join path space (\textbf{Challenge 3}). To materialize candidate PJ-views, the \textsc{join-graph-search} component uses a \textsc{Materializer}, a data processing component with the capacity to execute PJ queries.}

% \vspace{0ex}
% \end{tcolorbox}

\textsc{Join-Graph-Search} returns many \emph{candidate views}. Ranking the views is hard because of users' differing search criteria. The \textsc{view-distillation} component (line~\ref{dodline9}) summarizes the candidate views, further reducing the view search space as shown in \F\ref{fig:architecture}.

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize View Distillation (technical)}}]
      
% \vspace{-0ex}


\mypar{\textsc{View Distillation (technical)}} \emph{This component computes \emph{categories} from the candidate PJ-views that include redundancy and containment in the views, as well as opportunities for unioning views and more. Some categories can be used to distill/summarize the views (\textbf{Challenge 4}). Others are shared with the downstream component.}


\textsc{view-presentation} 
% (at the end of the funnel in \F\ref{fig:architecture}) 
receives the distilled views. It can \emph{rank} the views and return top-1 (for a full automated mode) or it can leverage the categories computed by \textsc{view-distillation} to help users find the right data (lines~\ref{dodline10}-\ref{dodline13}).

% ii) they guide the search for the desired output, which takes place within the \textsc{view-presentation} stage. The engine could \emph{rank} candidate PJ-views and return the top-1, concluding query processing. A challenge is in finding a relevant ranking criteria given the variety of user needs. Instead, our architecture 
% introduces a \textsc{signal-generation} component and a \textsc{view-presentation} stage (lines~\ref{dodline10}-\ref{dodline13}); both geared towards generating and using information efficiently to identify PJ-views. 

% \begin{tcolorbox} [
%       colframe=blue!25,
%       colback=white!10,
%       coltitle=blue!20!black,
%       right=0mm, left=0mm, bottom=0mm, top=1mm,
%       title={\textbf{\normalsize View Presentation (human)}}]
      
% \vspace{-0ex}

\mypar{\textsc{View Presentation (human)}} \emph{\textsc{View-presentation} uses different question interfaces to elicit information from users via data questions. The questions are designed to narrow down the space until users find the desired view (\textbf{Challenge 5}). The component chooses what questions to ask, sequentially, using a bandit-based approach.}

% The goal of view presentation is to help users select an adequate PJ-view. \sys{} employs a bandit-based approach which adaptively query the user and navigate the user to some adequate view. 

% \vspace{0ex}
% \end{tcolorbox}


Next, we present \textsc{View-Presentation} (Section \ref{sec:vpresentation}), \textsc{View-Distillation} (Section \ref{sec:vdistillation}).

% and the rest of \sys{}'s design in Section \ref{sec:engine}.












% \subsection{Component Description}

% We follow the lifecycle of query processing using the architecture in \F\ref{fig:architecture} that shows the \emph{human} components on the right-hand side and the engine's components in the enclosed dashed rectangle.

% \mypar{\textsc{View Specification} (human)} Users and programs use this component to define and submit queries to the system. Interfaces include Spreadsheet-style, API, natural language, and combinations of these. For QBE-based interfaces, the output of this stage is a set of example attributes and values. This specification can help reduce ambiguity in the search process by interacting with a knowledgeable user.

% \mypar{\textsc{Column Selection} (technical)} A component that analyzes the input query and identifies filter criteria to select a subset of relevant datasets from all available ones. This component must be designed to identify relevant data even when the input query is noisy, addressing \textbf{Challenge 1} above. The output of this component is a collection of candidate tables and columns.

% \mypar{\textsc{Discovery Index Creation} (technical) and \textsc{Engine} (technical)}
% The index creation works \emph{offline} to build discovery indexes over pathless table collections. This component must identify useful discovery indexes on pathless table collection. In particular, it needs to identify join paths (addressing \textbf{Challenge 2}) and other indexes used by the \textsc{column-selection} component. The Discovery engine provides \emph{online} access to the discovery indexes.


% \mypar{\textsc{Join Graph Search} (technical)} Given a set of candidate tables and an input query, this component identifies all possible join graphs that, when materialized, produce a candidate PJ-view. The main goal of this component is to address the large join path space (\textbf{Challenge 3}). To materialize candidate PJ-views, the join graph search component uses a \textsc{Materializer}, which is a data processing component with the capacity to execute PJ queries.

% \mypar{\textsc{Signal generation} (technical)} The engine produces many \emph{signals} while processing a query. The role of the \textsc{signal-generation} component is to collect, package, and offer these \emph{signals} to the \textsc{view- presentation} stage, hence helping reduce the number of candidate PJ-views, facilitating the presentation's job and thus addressing \textbf{Challenge 4}. 

% % We show in the next section how it is possible to reduce the size of the candidate PJ-views even before humans are involved by using this information carefully.

% \mypar{\textsc{View Presentation} (human)} The goal of view presentation is to help users select an adequate PJ-view. \sys{} employs a bandit-based approach which adaptively query the user and navigate the user to some adequate view.

% \smallskip

% In the following sections we present major components of our system, \textsc{View Presentation} (Section IV), \textsc{Signal Generation} (Section V), and its engine design and implementation (Section VI) including \textsc{Discovery Index Construction}, \textsc{Column Selection}, \textsc{Join Graph Search} and \textsc{Materializer}.

% \sys{} does not implement this component, but provides it with signals from \textsc{signal-generation}.
% To inform this component, Niffler's implementation focuses on providing signals that help navigate the space of PJ-views. 

% Given a collection of candidate PJ-views, the view presentation stage's goal is helping a consumer \zz{user or consumer?} select an adequate view. Due to the multiplicity of candidate PJ-views, this component must implement strategies to ease the navigation and selection of views even when the consumer (typically the same human who queries the system) does not have perfect knowledge of the target query. To ease the challenge, the architecture includes one more technical component which we explain next.\notera{raul: add citations to related work, view-summary(aditya), etc}



% \smallskip

% The main contribution of this paper is an implementation of the \emph{technical} components of the reference architecture, which we call Niffler, and present next.


==> sections/eval_setup.tex <==
\subsection{Datasets, and Setup}
\label{subsec:setup}

% \subsubsection{\textbf{Baselines}}

% To the best of our knowledge, there is no existing end-to-end system that focuses on finding PJ-views in a pathless scenario, as state of the art QBE systems are designed for settings where the exact schema is known a priori. We implement different baselines that include state of the art systems in their original form, and adapted to the pathless schema scenario.

% \mypar{Specification Baselines} \notera{explain the 3 modes that appear in the table and give them a name}

% \mypar{Search Baselines} \notera{we only have DoD, right? If so, then we need to explain here the attempt to run Squid standalone, and the lack of code for s4 and others}

% \mypar{Presentation Baselines} \notera{random (no intervention), TODO: search-ranking (however view search ranks results), s4-ranking (s4 ranking on top). Then, on top of the previous rankings, we apply view presentation.}

% \mypar{Data Discovery Baselines} \notera{we are running Aurum in 1 mode only. We may want to explore different modes to see how different parameters affect number of views, runtime, etc}

% \begin{table*}[ht]
% \begin{tabularx}{\linewidth}{|C|C|C|C|}
% \hline
%  & View Specification &   View Search  &   View Presentation \\ \hline
%  S4-pipeline& Choose all columns that contain at least one user example & \multirow{3}{10em}{ Explore join graphs using Aurum API and materialize all the views} & \multirow{3}{10em}{Use DoD view presentation strategies to find the ground truth view} \\ \cline{1-2}
%  Squid-pipeline& Choose columns that contain the most number of examples &                   &                   \\ \cline{1-2}
%  DoD-pipeline& Use clustering-based approach as described in \autoref{algo_cluster}&                   &                   \\ \hline
% \end{tabularx}
% \caption{end-to-end pipeline comparison \notera{as it stands, this table does not add much}}
% \label{tab:pipeline}
% \end{table*}





\subsubsection{Setup}

We run all experiments on a CentOS server with 128GB memory and a Intel(R) Xeon(R) CPU with 12 cores and 2.3GHz speed each. We built the reference implementation using python3.6. %\yg{Resolved}\notera{explain how it's implemented and its requirements.} 
The reference implementation requires configuring several parameters:

\begin{myitemize}

    \item \textbf{Similarity metric and threshold} The similarity metric and threshold needs to be set in Aurum to build the discovery index. We choose overlap similarity and set the threshold to be 0.8 in the evaluation. In \autoref{schema-quality}, we also experiment with modifying this threshold to study \textbf{RQ3}.
    
    \item \textbf{Maximum join hops} In the view search stage, we need to set the parameter $max\_hop$, which is the maximum number of join hops between tables. We set $max\_hop = 2$ on ChemBL and $max\_hop = 1$ on WDC, which suits the discovery needs well in practice.
    
    \zz{?}
    \item \textbf{Percentile for computing score threshold} We set the percentile, $p$, to be the 25-th percentile for computing the score threshold, $\tau$, during view presentation.
    
\end{myitemize}


==> sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we answer these research questions:
% evaluate \sys{}:

% In this section, we evaluate \textbf{\sys} from end to end in the same order we presented it. We first use a qualitative study to discuss state-of-the-art QBE systems. Then, a user study is performed to evaluate the end-to-end \sys{} pipeline for different queries (\textbf{RQ1}(human problem)). Last, we conduct an extensive quantitative evaluation on the other components of \sys{} (\textbf{RQ2}(4C algorithm), \textbf{RQ3}(the rest of the components)).

\begin{myitemize}


\item \textbf{RQ1}: Is \sys{} effective in navigating users to the view that satisfies their requirements? (human problem)

\item \textbf{RQ2}: Is \textsc{View-Distillation} useful for reducing the view choice space and is \textsc{View-Distillation} scalable? (technical problem)

\item \textbf{RQ3}: End-to-end evaluation of \sys{} (technical problem)

% \item \textbf{RQ3}: Do \textsc{column-selection} and \textsc{join-graph-search} find relevant PJ-views given a noisy input query over pathless table collections? (technical problem)

% \item \textbf{Microbenchmarks.} We explore the effect of various query and data parameters on \sys{}'s performance.

\item \textbf{Qualitative Study (QS).} We discuss qualitative differences with QBE systems.
% that were not designed for pathless table collections.

\end{myitemize}


\mypar{Datasets and Workload} We use three real-world large-scale datasets in the evaluation. Detailed statistics of these three datasets are shown in Table~\ref{tab:datasets}.

\begin{table}[ht]
\begin{center}
 \begin{tabular}{||c c c c c c||} 
 \hline
 Dataset & \#Tables & \#Columns & \specialcell{$\sim$\# Joinable\\ Columns} & \specialcell{$\sim$ Total\\ \#Rows} & Size\\ [0.5ex] 
 \hline\hline
 ChEMBL & 70 & 446 & 435 & 140M & 6.5GB\\ 
 \hline
 WDC & 10000 & 39939 & 11.6M & 140K & 45MB\\ 
 \hline
 Open Data & 69407 & 2955305 & 28.6M & 900M & 119GB\\
 \hline 
\end{tabular}
 \caption{Characteristics of Datasets}
 \label{tab:datasets}
\end{center}
\end{table}

\begin{myitemize}
    \item \textbf{ChEMBL}: ChEMBL~\cite{ChEMBL} is a database of bioactive molecules with drug-like properties. ChEMBL is large in terms of total data size. However, it has a relatively small number of tables and joinable columns.
    
    \item \textbf{WDC}: WDC is a subset of the web tables corpus~\cite{wdc} containing 10K tables crawled from the web. It has more than 10 million pairs of joinable columns.
    
    \item 
    \textbf{Open Data}~\cite{hu2019viznet}
    This dataset consists of 69K open datasets collected from the Open Data Portal Watch
    \cite{mitlohner2016characteristics,neumaier2016automated}\, which catalogs and monitors 262 open data portals such as NYC Open data, finances.worldbank.org, etc. %This repository consisted of around 69K tables with around 2.9 million columns and 0.9 billion rows.}
\end{myitemize}



\mypar{System Setup} We ran all experiments on a Ubuntu server with 500GB memory and an Intel(R) Xeon(R) CPU with 48 cores and 2.3GHz speed each. We built \sys{} using python3.6. \sys{} uses Aurum to find join paths without using schema information. 
% 's Jaccard Containment via the \textsc{Neighbors(threshold)} function with a threshold of 0.8---we experiment with other thresholds in Section~\ref{subsec:microbenchmarks}
In \textbf{ChemBL}, we ignore the schema information to simulate pathless scenario and instead use schema to evaluate ground truth.
When searching for join graphs, \sys{} uses by default a maximum of two hops, $\rho = 2$. We set the clustering threshold 
$\theta$ to 1, and the expected number of output views $k$ to be the total number of join graphs so we materialize all join graphs generated from \textsc{Join-Graph-Search}.

% \zz{maybe i missed it but i didn't see where did we specify $\theta$ (clustering threshold). is it still 1? and what about $\gamma$ (expected number of output views)? do we have a parameter for max num of hops?}


\subsection{RQ1: Is \sys{} effective in navigating users to the view that satisfies their requirements?\label{sec:userstudy}}

We conducted a within-subjects user study to answer this question. We give participants a task and expose them to two systems: \textsc{view-presentation} as explained in this paper, and a ranking of views as produced by overlap-based ranking mechanism of \topk{}~\cite{s4}. Their goal is to identify a view that satisfies the task.

\mypar{\textit{Participants}} We recruited 18 students with diverse backgrounds (CS, Economics, Math) from the University. We did not record any personally identifiable information.

\mypar{\textit{Study Procedure}} We design the study to ensure internal validity. Each participant attends a 30-min training session to learn the interface design. During the session, we describe the study, give a tutorial on each interface, and ask participants to solve two randomly-chosen \emph{trial} queries using \sys{} and \topk{}. The goal of the trial task is to familiarize participants with the interfaces. After finishing the trial tasks, each participant solves two different queries with \sys{} and \topk{}, respectively. The order in which the participant uses \sys{} and \topk{} is randomized to avoid ordering and learning effects. Participants work in isolation to avoid biasing each other. After finishing the tasks, participants answer a short survey about their experience with both systems. 

% We conducted a user study for answering this question. In the user study, we allow users to interact with \sys{}'s \textsc{view-presentation} and evaluate the effectiveness of the system to help users identify the desired view (\textbf{RQ1}). We recruited 18 participants with diverse backgrounds and asked them to answer two view discovery tasks using different strategies and later answered a survey to compare them. The two interface designs were a) \sys{}: The input examples are processed using \sys{} and the identified views are presented using Algorithm~\ref{algo_view_presentation}. b) \topk{}: The input examples are processed using the Select-All strategy of \topk{} and ranked based on the overlap of identified views with the input examples. The user iterates over the rank list to choose a view that satisfies the requirements specified in the input query. Each participant performed the task in isolation so that they do not bias other participants. In this evaluation, we compare the user responses to our survey and the quality of identified views to answer the following research questions.

%Through statistics collected from the user study, we have shown that \sys{}'s \textsc{view-presentation} implementation is better than \topk{}'s \textsc{view-presentation} implementation. 

% \mypar{\textit{Participant Information}} We recruited 18 students with diverse backgrounds (computer science, economics, math) from the University to participate. We did not record any personally identifiable information, and our study was exempted from the IRB.

\mypar{\textit{Task Setup}} Participants are exposed to 4 (2 trial, 2 study tasks) of the 5 queries shown in Table~\ref{tab:query_user_study} from WDC~\cite{wdc} dataset. We chose a diverse set of queries involving numerical and textual attributes that generated semantically ambiguous results.



\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    Query & Example & \specialcell{\sys{} \\ \#Views} & \specialcell{\topk{} \\ \#Views} \\\hline
       \specialcell{Find views containing\\ IATA code of airports\\in any of these states\\ in the US. }  &  \specialcell{Indiana, Georgia, \\ Virginia, Illinois,\\ Connecticut}  & 397 & 2255 \\ \hline
        \specialcell{Find views containing\\ churches in any of these\\ states in
the US} & \specialcell{Indiana, Georgia, \\Virginia, Illinois,\\
Connecticut} & 397 & 2255 \\ \hline
         \specialcell{Find views containing\\ newspaper companies in\\ any of these cities. } & \specialcell{San Diego,\\Boston,\\ Philadelphia} & 394 & 838\\ \hline
         \specialcell{Find views containing\\population of any of\\ these countries.} & \specialcell{China, Japan, \\United States} & 566 & 2235 \\ \hline
         \specialcell{Find views containing\\ the number of births \\per 1000 population\\in any of these countries.} & \specialcell{China, Japan,\\United States} & 566 & 2235 \\ \hline
    \end{tabular}
    \caption{Tasks used in the user study and \# Views generated by \sys{} / \topk{}.}
    \label{tab:query_user_study}
\end{table}

We manually verified each participant's output and record whether they found a relevant view that answers the query.

\mypar{\textit{Interface Setup}} We setup \sys{}'s \textsc{view-presentation} with different types of question interfaces. The interface asks users if they want to include a specific attribute, collection of attributes or an individual dataset (as discussed in Section~\ref{sec:vpresentation}). We use two different prioritization strategies for each interface: one based on the distance of the question from the input query and other based on the distance of the datasets corresponding to the questions from the input query. We use pre-trained word2vec embeddings to calculate distance. In each interaction, the user can either skip or answer the question or explore the ranking of views to select one view. The scoring model we adopted in \topk{} presents a ranking of views allowing the user to manually explore the options and pick the one that satisfies the input query.

%with \topk{} in the study. \topk{} proposes an efficient ranking algorithm to rank views based on their overlap with examples. We take the ranking of views as an implementation of \textsc{view-presentation} and refer to it as Ranking Interface. We refer to \sys{}'s \textsc{view-presentation} implementation as Question Interface.
%We feed examples of the five tasks to both \sys{} and \topk{} and get two sets of candidate views for each task. Then, we configure question interface with views generated by \sys{} and configure rank interface with views generated by \topk{}. 

\mypar{\textit{Data Collection and Results}} We log the interactions of each participant with the system for subsequent analysis. We measured interactions and outcomes to answer the following questions (Table~\ref{tab:userresult} presents the study results):

% The users answered the following questions after finishing both tasks.

% \begin{myenumerate}
% \item Can users find the ground truth datasets using \sys{} and \topk{}? Which interface do users prefer?
% \item How much time do users spend in view discovery?
% \item Is \sys{}'s view presentation intuitive and easy to follow?
% \end{myenumerate}

%In the system log, we recorded the following information automatically.
%\begin{myitemize}

 %   \item Does the user find a dataset in the end or end task without finding any dataset? 
  %  \item The time used to finish a task 
%    \item The number of questions answered before found a dataset (only for \sys{}). 
%\end{myitemize}

% \begin{myitemize}
%     \item \textbf{Q1} Does the user find the relevant view?
%     \item \textbf{Q2} Which system would you prefer to search datasets?
%     \item \textbf{Q3} If you are to forward the query and the dataset you chose using \sys{} (same question for \topk{}) to someone else. How confident are you to share the identified search result for the input query? 
%     \item \textbf{Q4} How difficult is to use \sys{}? 
%     \item \textbf{Q5} How difficult is to answer multiple choice questions with \sys{}? 
    
% \end{myitemize}


% \mypar{\textit{Results}} 

% \notera{order questions in table based on this order}

\noindent\underline{Q1. Does the user find the relevant view?} $16/18$ participants identify the correct view with \sys, versus only $6$ when using the \topk{} ranking. $12$ participants finished the task without finding any dataset using \topk{} versus only $1$ with \sys{}. The results are statistically significant: we run Fisher's exact test and obtain a p-value of $0.002$. Due to this result, we confirm the sample size is adequate for this study.

\noindent\underline{Q2. Which system would you prefer to search datasets?} $12$ participants prefer searching for datasets with \sys{} and $5$ prefer \topk{} (1 participant was not sure).

% Using \sys{}, $16$ individuals correctly identified a view that satisfies the requirements of the input query, $1$ individual ended the task without finding any dataset that satisfied the query and $1$ individual chose an incorrect dataset. In contrast, only $6$ participants identified a relevant view with \topk{} and $12$ individuals ended the task without finding any dataset. \notera{spell out the hypothesis}We ran a fisher exact test to evaluate the statistical significance of this result, and it returned a p-value of $0.002$. 

% Participants' ability to search with \sys{} is also reflected in $12$ participants preferring the \sys{} interface  as compared to $5$ individuals liking the \topk{} interface and $1$ individual was unsure about their preference. One peculiar property we noticed is that queries $3$ and $5$ are the only queries where participants prefer \topk{} because the required view is ranked among the top $10$ datasets. All other queries are difficult to answer using \topk{} as the required view is not present in top 30 views.

\noindent {Q3. If you are to forward the query and the dataset you chose} using \texttt{\textbf{Ver}} same question for \textsc{FastTopK}) to someone else. \underline{How confident are you to share the identified search result} \underline{ for the input query?} $14$ participants were confident with the result they found with \texttt{\textbf{Ver}}. We cannot measure confidence for \textsc{FastTopK} because 12 participants did not find any view.

% We compared the confidence of participants in the output of \sys{} and \topk{}. The results for \topk{} are not conclusive because $66.67\%$ individuals could not identify the required view and had to end the task. For \sys{}, $14$ participants ($77.77\%$ individuals) mentioned that they are confident about the identified dataset.

\noindent\underline{Q4. How difficult is to use \texttt{\textbf{Ver}}}? and {Q5. How difficult is to }  {answer multiple choice questions with \texttt{\textbf{Ver}}?} $14$ participants deemed using \sys{} easy and intuitive and $4$ disagreed. Anecdotally, some participants mentioned that questions asked by \sys{} are easy to answer and do not require in-depth analysis.
Our discussion with the participants revealed that different users preferred different interface designs. For example, some students verified the attribute names before choosing a view while others verified a sample of the records.

\noindent\underline{Time taken} The median participant using \sys{} finds the view within 101 seconds (median) and with a median of $3$ interactions. They take 93 seconds (median) when using \topk{}.

% Majority of the participants identify the required view using \sys{} in less than 101 seconds (with less than $3$ median number of interactions). The participants spend a similar amount of time with \topk{} (median time is 93 seconds) to search for the required view. This shows that \sys{} helps to efficiently identify the required view and requires very few interactions in the search process. 





\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\rowcolor{LightCyan}
\multicolumn{3}{|c|}{\specialcell{ Q1. Does the user find a relevant view?}} \\ \hline \hline
& \sys{} & \topk{} \\ \hline
Found & $\textbf{16}^*$ & 6 \\ \hline
Not Found & 2 & 12 \\ \hline 
\multicolumn{3}{|c|}{\specialcell{*Result is statistically significant with  p-value of 0.002}} \\ \hline \hline
\rowcolor{LightCyan}
\multicolumn{3}{|c|}{\specialcell{ Q2. Which system would you prefer to search datasets?}} \\ \hline \hline
\sys{}     &  \topk{} & Unsure \\ \hline
\textbf{12}     &  5 & 1 \\ \hline
\hline
\rowcolor{LightCyan}
\multicolumn{3}{|c|}{\specialcell{ Q3. Confidence in the identified search result}} \\ \hline \hline
& \sys{} & \topk{} \\ \hline
Confident & \textbf{14} & 6 \\ \hline
Not Confident & 4 & 8 \\ \hline
\hline
\rowcolor{LightCyan}
\multicolumn{3}{|c|}{\specialcell{  Q4. How difficult is to use Ver?}} \\ \hline \hline
\multicolumn{2}{|c|}{Intuitive}   & Not Intuitive \\ \hline
\multicolumn{2}{|c|}{\textbf{14}} & 4 \\ \hline \hline
\rowcolor{LightCyan}
\multicolumn{3}{|c|}{\specialcell{ Q5. How difficult is to answer multiple choice questions with Ver?}}            \\ \hline \hline
\multicolumn{2}{|c|}{Easy}      &  Difficult \\ \hline 
\multicolumn{2}{|c|}{\textbf{16}}     &  2 \\ \hline
\end{tabular}
\caption{Summary of survey results. \label{tab:userresult}}
\end{table}

%\yg{@sainyam xx is the placeholder for actual data. could you fill in those?} We first analyze the data collected from system log. Using \sys{}, $16$ participants found satisfactory datasets and two could not find any dataset for the input query. Using \topk{}, $6$ participants found satisfactory datasets and $12$ did not find any. We also compare the time used in each system to finish a task. In \sys{}, the median of time used to finish a task is $101$ seconds, while in \topk{}, the median is $93$ seconds. From these two statistics, we can conclude that given comparable exploration time, \sys{} is more effective in helping users find a satisfactory dataset than \topk{}. Besides, the number of questions answered before found a dataset in \sys{} is $3$, which shows the \textsc{view-presentation} of \sys{} is efficient in terms of the interaction needed from users. \yg{not sure if we can argue this since we do not have another baseline using interaction model. in other words, we do not know how small is small for interaction number}

%Next, we will analyze the data collected from user survey. For Q1, xx users think learning the use of Question Interface is intuitive, xx think it is unintuitive. For Q2, xx users rate the difficulty to answer multiple choice questions of \sys{} as easy, xx rate it as difficult. For Q3, xx participants choose \sys{}, xx choose \topk{} and xx choose 'unsure'. We report the result of Q4 and Q5 in Table \ref{tab:survey}.


% \subsection{Experimental Setup}

% \subsubsection{Noisy User Workload}

% The workload consists of a collection of 2-column, %\zz{reviewer1 W3: all the experiments are evaluated on 2-col examples. However, it is not discussed on whether "2-col" examples are sufficient to practical cases. FIX: we can explain we have 5.5.3 to vary number of columns later in the paper.}
%  3-row example queries and we experiment with varying number of rows and columns in Section~\ref{subsec:microbenchmarks}. %\zz{reviewer3 D7: Why only 5 queries, and why only 2 columns and 3 rows (is this a standard choice/assumption for QBE systems)? FIX: second comment that missed the 5.5.3 experiment. Let's make sure we explain we explore more columns in the microbenchmarks.}
% To generate the workload, we first find a PJ-query that produces a result we call the \emph{ground truth PJ-view}. Columns in the \emph{ground truth PJ-view} are called \emph{ground truth columns}. Then, we generate the $2\times 3$ input queries according to three strategies, \emph{Zero Noise}, \emph{Medium Noise}, and \emph{High Noise}. \emph{Zero noise} means we sample values from the \emph{ground truth columns}. In \emph{Medium noise} we sample $\frac{2}{3}$ values from the \emph{ground truth columns} and $\frac{1}{3}$ from a \emph{noise column}, which is a column with a Jaccard Containment of more than 0.8 with respect to the \emph{ground truth column}. Finally, in \emph{High noise} we sample $\frac{1}{3}$ values from the \emph{ground truth column} and $\frac{2}{3}$ from the \emph{noise columns}.


% \subsubsection{Datasets and Workload}

% We use 2 real-world large-scale datasets in the end-to-end evaluation. Detailed statistics of these two datasets are shown in Table~\ref{tab:datasets}.

% \begin{table}[ht]
% \begin{center}
%  \begin{tabular}{||c c c c c||} 
%  \hline
%  Dataset & \#Tables & \#Columns & \specialcell{\#Approx.\\Joinable\\ Columns} & \specialcell{Avg\\ \#Rows }\\ [0.5ex] 
%  \hline\hline
%  ChEMBL & 70 & 446 & 435 & 2 million\\ 
%  \hline
%  WebTable & 10000 & 39939 & 11.6 million &  14\\ 
%  \hline 
% \end{tabular}
%  \caption{Characteristics of Datasets}
%  \label{tab:datasets}
% \end{center}
% \end{table}


% \begin{myitemize}
%     \item \textbf{ChEMBL}: ChEMBL~\cite{ChEMBL} is a database of bioactive molecules with drug-like properties. ChEMBL is large in terms of total data size. However, it has a relatively small number of tables and joinable columns.
    
%     \item \textbf{Web Tables}~\cite{wdc} data collection is a subset of the WDC corpus containing 10K tables crawled from the web. It has more than 10 million pairs of joinable columns. 
% \end{myitemize}

% We generate 5 ground truth queries by sampling join paths from the ground truth views of each dataset, 5 noisy user queries (consisting of example values) for each ground truth view and for each of the 3 noise levels. This results in a total of 150 noisy user queries across both datasets and noise levels.

% \subsubsection{Setup}

% We run all experiments on a CentOS server with 128GB memory and an Intel(R) Xeon(R) CPU with 12 cores and 2.3GHz speed each. We built the reference implementation using python3.6. The reference implementation uses Aurum as the implementation of the \textsc{Discovery-Index-Construction} and \textsc{Discovery Engine}. \sys{} uses Aurum's Jaccard Containment via the \textsc{Neighbors(threshold)} function with a threshold of 0.8---we experiment with other thresholds in Section~\ref{subsec:microbenchmarks}. When searching for join paths, \sys{} uses by default a maximum of two hops \zz{maybe i missed it but i didn't see where did we specify $\theta$ (clustering threshold). is it still 1? and what about $\gamma$ (expected number of output views)?}.

% column retrieval and join path search

\input{sections/rq2}
\input{sections/4c_scalability}

\input{sections/comparison}

\input{tables/sota-components}

\input{sections/qualitative_qbe}


% signal generator
% \input{sections/rq3} 




% microbenchmarks
% \input{sections/microbenchmarks}



==> sections/generalization_table.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Query &
  \begin{tabular}[c]{@{}c@{}}View-Spec\\ Implementation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Original\\ \#Views\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\#Views After\\ Pruning\end{tabular} \\ \hline
\multirow{3}{*}{1618} & Keyword   & 380   & 380   \\ \cline{2-4} 
                      & Attribute & 1043  & 1043  \\ \cline{2-4} 
                      & QBE       & 27562 & 12017 \\ \hline
\multirow{3}{*}{1325} & Keyword   & 260   & 260   \\ \cline{2-4} 
                      & Attribute & 881   & 881   \\ \cline{2-4} 
                      & QBE       & 170   & 86    \\ \hline
\multirow{3}{*}{1863} & Keyword   & 155   & 155   \\ \cline{2-4} 
                      & Attribute & 1030  & 1030  \\ \cline{2-4} 
                      & QBE       & 5441  & 3074  \\ \hline
\multirow{3}{*}{340}  & Keyword   & 2     & 2     \\ \cline{2-4} 
                      & Attribute & 730   & 730   \\ \cline{2-4} 
                      & QBE       & 2     & 2     \\ \hline
\multirow{3}{*}{42}   & Keyword   & 620   & 613   \\ \cline{2-4} 
                      & Attribute & 41    & 36    \\ \cline{2-4} 
                      & QBE       & 541   & 55    \\ \hline
\multirow{3}{*}{1504} & Keyword   & 192   & 169   \\ \cline{2-4} 
                      & Attribute & 2     & 2     \\ \cline{2-4} 
                      & QBE       & 5619  & 859   \\ \hline
\multirow{3}{*}{1577} & Keyword   & 9     & 9     \\ \cline{2-4} 
                      & Attribute & 11    & 11    \\ \cline{2-4} 
                      & QBE       & 4791  & 4467  \\ \hline
\multirow{3}{*}{1824} & Keyword   & 175   & 174   \\ \cline{2-4} 
                      & Attribute & 1     & 1     \\ \cline{2-4} 
                      & QBE       & 93    & 7     \\ \hline
\multirow{3}{*}{679}  & Keyword   & 102   & 102   \\ \cline{2-4} 
                      & Attribute & 11    & 11    \\ \cline{2-4} 
                      & QBE       & 7878  & 7862  \\ \hline
\multirow{3}{*}{859}  & Keyword   & 295   & 295   \\ \cline{2-4} 
                      & Attribute & 1043  & 1043  \\ \cline{2-4} 
                      & QBE       & 465   & 241   \\ \hline
\end{tabular}
\caption{\update{}{Original number of views, and number of views after pruning compatible and contained views using different implementations of View-Specification}}
\label{tab:view-spec-alternative}
\end{table}

==> sections/implementation.tex <==
\section{\sys{} Design and Implementation}
\label{sec:engine}

%\zz{reviewer1 W1: most of the components in Section 4 utilize existing methods or derive from existing approaches with some modifications. FIX: We could say this upfront and insist that the contribution is the architecture. And that the architecture is a contribution because it allows us to work on problems at a scale much larger than other QBE systems, despite the harder scenario we target.}

% We introduce next the remaining components of the reference architecture that constitute \sys{}.

% In this section, we introduce \sys{}, which we use to make the reference architecture precise and evaluate it later. Thus, in implementing \sys{}, we reuse components and techniques from the literature when possible and explain novel design and implementation decisions when relevant.

% \new{In this section, we explain the implementation details of \dod. \dod's main contribution \emph{is not} in the implementation of any one component, whose implementation we adapt from the literature. Instead, the contribution is in the way we combine those components together according to the reference architecture, which makes \dod scale to larger (more data) and harder (pathless table collections) problems than existing solutions.}

\subsection{Discovery Index Construction}

\sys{} leverages Aurum~\cite{aurum} to efficiently build a discovery index over large collections of data. \sys{} uses the following functions provided by Aurum:

% This component identifies approximate join paths on pathless table collections, and through a \textsc{Discovery Engine} (see \F\ref{fig:architecture}) retrieves data that satisfies a query filter. In this paper, we use Aurum~\cite{aurum}, which we briefly introduce here for completeness. During an offline stage, Aurum reads each $D\in \mathcal{D}$ and produces a \emph{profile} for each column in $D$. The profile includes common statistics as well as sketches, constructed specifically to identify relationships between columns and tables. After reading the data once, Aurum produces a full-text search index over attributes and data values, and a hypergraph. In the hypergraph, nodes represent columns, hyperedges represent columns of the same table. Edges are directed and weighted. Each relationship is represented with a different edge type. The hypergraph is constructed efficiently (\eg no all-pairs comparison are involved) using LSH-based indexes for the relationships of interest, which in this paper are \emph{content-similarity}, and \emph{inclusion-dependency}~\cite{fernandez2019lazo}. 
% The \textsc{Discovery Engine} provides the following primitives:

\mypar{\textsc{Search-Keyword(target, fuzzy)}} Given an input string, it returns columns that contain the string in either the attribute name, or in the values, as specified by \textsc{target}. The match can be exact or fuzzy, after specifying a maximum Levenshtein distance.

\mypar{\textsc{Neighbors(threshold)}} Given an input column, it returns all neighbors with a Jaccard containment~\cite{fernandez2019lazo} above the input \textsc{threshold}.

\mypar{\textsc{Generate-Join-Graphs(tables, $\rho$)}} Given a set of tables, it returns all join graphs connecting input tables, via inclusion dependencies. Each edge in the join graph has a maximum number of hops, $\rho$.


\subsection{Column Selection}

\textsc{Column-Selection} generates a set of columns $\textsc{Cand}(A_i)$ given user-provided input examples, $\chi.A_i$. To deal with noisy inputs, the component clusters candidate columns and returns clusters with top-$\theta$ scores. Setting $\theta=1$ returns clusters with the highest overlap with $\chi.A_i$ (there could be ties). In contrast, $\theta=\infty$ returns any column with non-empty overlap. This relaxed design makes the component more robust to noisy inputs than methods based on \emph{exact containment}~\cite{squid,duoquest}, and more efficient than methods based on \emph{non-empty containment}.

% Given a column of example values as input ($\chi.A_i$), this component generates a small set of columns $\textsc{Cand}(A_i)$ that contain these values. Our implementation supports textual and categorical columns. Many QBE systems~\cite{squid,duoquest} follow the strict assumption that only the columns containing all example values are considered as candidates for subsequent stages of the pipeline (\textit{exact containment}). However, the noisy QBE-style query may not contain all values from the ground truth PJ-view (Challenge 1), thereby affecting its ability to identify adequate PJ-views. In contrast, a relaxed approach to construct $\textsc{Cand}(A_i)$ is to enumerate all columns that have a non-empty overlap with the input examples (\textit{non-empty containment}). This approach ensures that the ground truth view is always present in $\textsc{Cand}(A_i)$ but is highly inefficient when a token is present in several tables. Our \textsc{column-selection} algorithm provides the flexibility to vary the strictness of the assumption by grouping columns identified by relaxed methodology and selecting the top $\theta$ (an input parameter) clusters for the subsequent components. Varying the value of $\theta$ simulates varying degrees of strictness. For example, $\theta=1$ is equivalent to considering the cluster that contains the column having maximum overlap with the input example whereas $\theta=\infty$ considers all columns that have non-empty overlap with the input examples. The identified clusters help to summarize the set of candidate columns $\textsc{Cand}$ and prioritize the clusters in non-increasing overlap with input examples. Through clustering similar columns and selecting relevant columns based on clusters, our \textsc{column-selection} is more error-tolerant than methods based on \textit{exact containment} and more efficient than methods based on \textit{non-empty containment}.

\IncMargin{1em}
\begin{algorithm}\SetKwFunction{Union}{Union}
\scriptsize
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\Input{Example value set $\chi.A_i$ for a column $A_i$, Discovery Index $I$, Clustering threshold $\theta$  } 
	\Output{$\textsc{Cand}(A_i)$ Candidate columns and scores.}
	 \BlankLine 
	 
	 $\textsc{Cand}(A_i) \leftarrow \phi$\\% \tcc*[f]{\small Initialize candidates}\\
	 	 \For{ $e\in \chi.A_i$ \label{crline2}}
	 {
	    
	    $\textsc{Cand}(e) \leftarrow \textsc{Search-Keyword}(e)$\\
	    %\tcc*[f]{\small Query Discovery engine to get all columns containing the example value $e$}\\
	 	$\textsc{Cand}(A_i) \leftarrow \textsc{Cand}(A_i) \cup \textsc{Cand}(e)$\label{crline4}
	 }
	 
	 $ \mathcal{C} \leftarrow \textsc{Connected-Component}(\textsc{Cand}(A_i), I)$\label{crline5}\\ %\tcc*[f]{\small Cluster candidate columns using connected component algorithm}\\
	 \For{ $Cluster\in \mathcal{C}$ }{
% 	 \tcc*[h]{Score clusters based on overlap}\\
	    $\textsc{Score}(Cluster) = \max_{col\in Cluster} (| col \cap \chi.A_i |) \label{crline7} $
	 }
	 $\mathcal{C}'\leftarrow$ top-$\theta$ clusters in $\mathcal{C}$ based on $\textsc{Score}$\label{crline8}\\
	 $\textsc{Cand}(A_i) \leftarrow \bigcup_{T\in \mathcal{C}'} T$\\%\tcc*[f]{\small Combine all columns in top-$\theta$ clusters}\\
	 \Return $\textsc{Cand}(A_i)$
 	 	  \caption{\textsc{Column-Selection}}
 	 	  \label{algo_column_retrieval} 
 	 \end{algorithm}

\noindent\textbf{Algorithm}~\ref{algo_column_retrieval} presents the \textsc{column-selection} algorithm. First, it identifies all columns that have a non-empty overlap with the input examples (lines~\ref{crline2}-\ref{crline4}). These columns are then clustered by finding connected components over the hypergraph constructed by the \textsc{discovery engine} (line~\ref{crline5}). To identify the connected components, it uses the discovery \textsc{Neighbors} function. Each cluster is assigned a score that corresponds to the maximum number of examples contained in any column in the cluster (line~\ref{crline7}). This stage supports both \textit{automatic mode} and \textit{interactive mode}. In the \textit{automatic mode}, top-$\theta$ clusters are selected based on their scores (line~\ref{crline8}). 

\mypar{Rationale} Isolating this component in the architecture has two advantages: i) it detects ill-specified queries that lead to too many unnecessary retrieved columns; ii) it offers a point of interaction with \textsc{view-specification} to help users select the right column clusters. Identifying interactive policies to present clusters is outside the scope of this work; we focus on providing the mechanism.


\subsection{Join Graph Search and Materializer}

The \textsc{Join-Graph-Search} and \textsc{Materializer} components construct candidate PJ-views by joining the tables returned by \textsc{column-selection}. The pseudocode in Algorithm~\ref{algo_view_search} operates in two steps. 

% First, \textbf{Join Graph Enumeration} (lines~\ref{vsline1}-\ref{vsline10}) enumerates all columns returned by \textsc{column-selection}, identifies joinable groups of their corresponding tables and find all join graphs in a joinable group. Second, the \textbf{Ranking and Materialization} (lines~\ref{vsline11}-\ref{vsline12}) component ranks these join graphs based on their quality estimated by the \textsc{discovery-engine} and materializes the top-$k$ join graphs.

% \begin{myenumerate}

\noindent\underline{1) Join Graph Enumeration (lines~\ref{vsline1}-\ref{vsline10})} enumerates all possible combinations of the columns returned by \textsc{column-selection}, identifies joinable groups of their corresponding tables and find all join graphs in a joinable group. A join graph consists of a group of columns connected via join paths. Given a pair, $c_i, c_j$, of non-joinable columns, no combination of columns involving $c_i$ or $c_j$ can be joined. Non-joinable pairs are cached to skip computation.

% These candidates are then processed to iteratively remove the combination which can not be constructed by joining tables through the constructed index. Note that if columns $c_i$ and $c_j$ can not join then any combination of columns involving $c_i$ and $c_j$ can not be joined. This phase uses this optimization along with a cache to efficiently prune out incorrect combinations.

\noindent\underline{2) Ranking and Materialization (lines~\ref{vsline11}-\ref{vsline12})} materializes the top-$k$ views as ranked according to the discovery engine score. The discovery engine ranks views according to how well join graphs approximate PK/FK, and according to the size of the join graph; smaller graphs rank higher. Views are materialized incrementally via a materializer built on top of Pandas~\cite{pandas}; it can be adapted to use an embedded database~\cite{sqlite, duckdb} or a processing engine with the \emph{external table} feature~\cite{redshiftexternal} to achieve better performance. 

% \noindent2) Ranking and Materialization ranks the join graphs based on the join score generated by the \textsc{discovery engine} and then materializes the top-$k$ views. The intuition of the scoring model in \textsc{discovery engine} is that a good join graph needs to have join keys that are more likely to be PK/FK and involves fewer tables. Our \textsc{discovery engine} collects data of these two criteria and assigns a score to each join graph. Note that our ranking strategy is efficient since it can be calculated without materializing the views. Given the ranking information, we can materialize the top-$k$ views. Besides, we also support materializing join graphs in \textit{batch} mode. Through avoiding materializing all the views at once, we alleviate the scalability issue when the number of join graphs is large. The materializer is built on top of Pandas~\cite{pandas} and could use an embedded database~\cite{sqlite, duckdb} or a processing engine with the \emph{external table} feature~\cite{redshiftexternal} to achieve better performance. 
    
% \end{myenumerate}

\begin{algorithm}
\scriptsize
\SetKwFunction{AllCombinationOf}{AllCombinationOf} \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	
	\Input{QBE-style query $\chi$, candidate columns $\textsc{Cand}$,
	expected number of output views $k$
	} 

	\Output{$\mathcal{V}_{PJ}$: list of candidate PJ-views}
	\tcc*[h]{Step 1: Join Graph Enumeration}\\
	$\tau\leftarrow |\textsc{Columns}(\chi)|$\label{vsline1}\\%\tcc*[f]{Number of columns in input examples}
% 	\tcc*[h]{Get source table of each column}\\
% 	$\textsc{Cand\_Table}(A_i) \leftarrow \{col_i.get\_table(): \forall col_i\in \textsc{Cand}(A_i)\}$ \\
	$\Gamma\leftarrow \{(c_1,\ldots, c_\tau): \forall c_i\in \textsc{Cand}(A_i)\}$ \\%\tcc*[f]{Construct all combinations of columns} \\%\zz{reviewer3 D4: I'm not sure I get the notation in Line 2 of Algorithm 3, is that correct?}\\
	%\sg{Above line has exponential complexity}\\
	$\Gamma_{join}\leftarrow \phi$\\
	 \For{ $r\equiv (c_1,\ldots, c_\tau) \in \Gamma$}
	 {
	 \tcc*[h]{Get join graphs  between source tables of $r$ with $\rho=2$}\\
	 $P\leftarrow
	 \textsc{Generate-Join-Graphs}(r.tables(),2)$ \\
	 \If{$\exists c_i,c_j \in r \mid P(c_i,c_j) = \phi$}{
	    Remove all candidates $r\in \Gamma$ containing columns $c_i$ and $c_j$ such that $P(c_i,c_j)=\phi$  \\%\tcc*[f]{Prune out combinations that do not have a join path}\\
	    Continue\\ 
	 }\Else{
	    $\Gamma_{join}\leftarrow \Gamma_{join} \cup  P$\label{vsline10}
	 }
	 }
	 \tcc*[h]{Step 2: Ranking and Materialization}\\
	 $\Gamma_{join}'\leftarrow $ Select top $k$ join candidates based on join score generated by the discovery engine.\label{vsline11}\\
	 $\mathcal{V}_{PJ}\leftarrow \textsc{materialize-views}(\Gamma_{join}')$\label{vsline12}\\
	
	\Return $\mathcal{V}_{PJ}$
    \caption{\textsc{Join-Graph-Search}}
 	\label{algo_view_search} 
\end{algorithm}




==> sections/old/_rq2.tex <==
\subsection{RQ2: Effect of Pathless Schema Quality}
\label{schema-quality}





% \begin{figure*}
%   \centering
%   \includegraphics[width=\linewidth]{figures/presentation/chembl/time.png}
%   \caption{ChemBL: total running time of end-to-end pipelines}
%   \label{fig:chembl-total-time}
% \end{figure*}

% \begin{figure*}
%   \centering
%   \includegraphics[width=\linewidth]{figures/presentation/wdc/time.png}
%   \caption{WDC: total running time of end-to-end pipelines}
%   \label{fig:wdc-total-time}
% \end{figure*}


==> sections/old/eval.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we address four points including the main research questions of the paper \textbf{RQ1} and \textbf{RQ2}:

\begin{myitemize}

\item \textbf{Qualitative Study (QS).} State-of-the-art QBE systems over pathless table collections
\item \textbf{RQ1}: Do \textsc{column-selection} and \textsc{join-graph-search} find relevant PJ-views given a noisy input query over pathless table collections? 
\item \textbf{RQ2}: Are the 4C-based signals useful for reducing the view choice space?
\item \textbf{Microbenchmarks.} We explore the effect of various query and data parameters on Niffler's performance.

    
\end{myitemize}

Niffler is built to solve the technical problem and not the human problem of PPE. Consequently, the research questions focus on measuring the degree to which the engine helps identify relevant PJ-views over pathless table collections given a notion of PJ-view.

% The research questions focus on evaluating the degree to which the engine helps identify relevant PJ-views over pathless table collections given a notion of relevant PJ-view. 
% In particular, we do not solve the problem end-to-end. That requires humans to tune input queries in the \textsc{view-specification} stage and to resolve semantic ambiguity in the \textsc{view-presentation} stage. Implementing these components is a challenge that requires designing the user interaction. 
\subsection{User study}
\yg{discuss: I argue here the goal is to show niffler is an effective approach for assisting users in the view discovery process, but we do not really let users experience the whole system}

In the user study, our goal is to answer if Niffler is an effective approach for assisting users in the view discovery process. We recruit 18 participants with various backgrounds and ask them to finish a few view discovery tasks using different view discovery interfaces. Through statistics collected from the user study, we are able claim that \yg{to add}

\subsubsection{Participant} We invite 18 students with various backgrounds (computer science, economics, math) from the department building.

\subsubsection{Task Setup} We choose five view discovery tasks.
\yg{add five queries}

\subsubsection{System Configuration}
We configure our reference architecture with two different implementations. The first one is Niffler implementation.
\yg{If we want to make user study the first section in the evaluation, we need to introduce S4 here}
\begin{itemize}
    \item Niffler: \textsc{Column-Selection} $\rightarrow$ Join-Graph-Search $\rightarrow$ Signal-Generation $\rightarrow$ View-Presentation
    \item Baseline:
    \textsc{SELECT-ALL} $\rightarrow$ Join-Graph-Search $\rightarrow$ S4 Ranking
\end{itemize}

\subsubsection{Interface Setup}
\yg{add interface description, figures ...}
\subsubsection{Study Procedure}
\subsubsection{Data Collection}
\subsubsection{Data Analysis}

\subsection{Experimental Setup}

\subsubsection{Noisy User Workload}

The workload consists of a collection of 2-column, %\zz{reviewer1 W3: all the experiments are evaluated on 2-col examples. However, it is not discussed on whether "2-col" examples are sufficient to practical cases. FIX: we can explain we have 5.5.3 to vary number of columns later in the paper.}
 3-row example queries and we experiment with varying number of rows and columns in Section~\ref{subsec:microbenchmarks}. %\zz{reviewer3 D7: Why only 5 queries, and why only 2 columns and 3 rows (is this a standard choice/assumption for QBE systems)? FIX: second comment that missed the 5.5.3 experiment. Let's make sure we explain we explore more columns in the microbenchmarks.}
To generate the workload, we first find a PJ-query that produces a result we call the \emph{ground truth PJ-view}. Columns in the \emph{ground truth PJ-view} are called \emph{ground truth columns}. Then, we generate the $2\times 3$ input queries according to three strategies, \emph{Zero Noise}, \emph{Medium Noise}, and \emph{High Noise}. \emph{Zero noise} means we sample values from the \emph{ground truth columns}. In \emph{Medium noise} we sample $\frac{2}{3}$ values from the \emph{ground truth columns} and $\frac{1}{3}$ from a \emph{noise column}, which is a column with a Jaccard Containment of more than 0.8 with respect to the \emph{ground truth column}. Finally, in \emph{High noise} we sample $\frac{1}{3}$ values from the \emph{ground truth column} and $\frac{2}{3}$ from the \emph{noise columns}.


\subsubsection{Datasets and Workload}

We use 2 real-world large-scale datasets in the end-to-end evaluation. Detailed statistics of these two datasets are shown in Table~\ref{tab:datasets}.

\begin{table}[ht]
\begin{center}
 \begin{tabular}{||c c c c c||} 
 \hline
 Dataset & \#Tables & \#Columns & \specialcell{\#Approx.\\Joinable\\ Columns} & \specialcell{Avg\\ \#Rows }\\ [0.5ex] 
 \hline\hline
 ChEMBL & 70 & 446 & 435 & 2 million\\ 
 \hline
 WebTable & 10000 & 39939 & 11.6 million &  14\\ 
 \hline 
\end{tabular}
 \caption{Characteristics of Datasets}
 \label{tab:datasets}
\end{center}
\end{table}


\begin{myitemize}
    \item \textbf{ChEMBL}: ChEMBL~\cite{ChEMBL} is a database of bioactive molecules with drug-like properties. ChEMBL is large in terms of total data size. However, it has a relatively small number of tables and joinable columns.
    
    \item \textbf{Web Tables}~\cite{wdc} data collection is a subset of the WDC corpus containing 10K tables crawled from the web. It has more than 10 million pairs of joinable columns. 
\end{myitemize}

We generate 5 ground truth queries by sampling join paths from the ground truth views of each dataset, 5 noisy user queries (consisting of example values) for each ground truth view and for each of the 3 noise levels. This results in a total of 150 noisy user queries across both datasets and noise levels.

\subsubsection{Setup}

We run all experiments on a CentOS server with 128GB memory and an Intel(R) Xeon(R) CPU with 12 cores and 2.3GHz speed each. We built the reference implementation using python3.6. The reference implementation uses Aurum as the implementation of the \textsc{Discovery-Index-Construction} and \textsc{Discovery Engine}. Niffler uses Aurum's Jaccard Containment via the \textsc{Neighbors(threshold)} function with a threshold of 0.8---we experiment with other thresholds in Section~\ref{subsec:microbenchmarks}. When searching for join paths, Niffler uses by default a maximum of two hops.


\input{sections/comparison}

% column retrieval and join path search
\input{sections/rq1}

% signal generator
\input{sections/rq3} 

\input{sections/sota-components}

% microbenchmarks
\input{sections/microbenchmarks}



==> sections/old/implementation.tex <==
\section{Engine Design and Implementation}
\label{sec:dod}

In this section, we explain the implementation details of \dod. Our design follows the reference architecture and we propose novel algorithms for the different components of the architecture.

\sg{Add overall pseudo code for \dod}

% Dataset-on-Demand's architecture consists of three \emph{stages} that address the challenges above. We build DoD on top of Aurum~\cite{aurum}, a data discovery system.

%To address the challenges of finding relevant columns/tables, exploring join paths and navigate users to their preferred views, we build an end-to-end system which consists of three conceptually independent stages that work seamlessly to deliver the final views: view specification, view search and view presentation. \autoref{fig:pipeline} depicts DoD's end-to-end pipeline.

%We build the three stages of DoD on top of Aurum \cite{aurum}, an open source data discovery platform.

% \textbf{Aurum overview.} Aurum reads relations from data sources such as databases, lakes, and files in filesystems, and produces a discovery index (corresponds to step 0 in Fig. 1).
% DoD uses Aurum's discovery index to understand what columns are similar to each other, and to understand inclusion dependencies. Aurum finds these relationships in a scalable manner at the cost of introducing false positives. DoD handles this uncertainty with the help of users.
%The discovery index is logically a hypergraph where the nodes correspond to columns and edges represent relationships (e.g.inclusion dependency) between columns. Based on this hypergraph, Aurum provides an API to query join paths between two tables. Additionally, the discovery index also includes a full text search index of textual columns and their attribute names. Based on the full text search index, Aurum provides an API to query relevant columns that contain certain values.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/overview.png}
%   \caption{DoD's end-to-end pipeline: Step 0: Aurum builds a discovery index from a collection of tables. Step 1: A user creates and submits a query view. Step 2: DoD searches for relevant columns using Aurum API (\textit{Q1}) and cluster them based on content similarity. Step 3(Optional): DoD presents column clusters to the user and let the user choose desired clusters. Step 4: DoD explores all join paths through Aurum discovery index (\textit{Q2}), ranks all join paths and provide materialized views to the next stage. Step 5: DoD applies 4C method to result views and user interacts with the presentation framework.}
 
%   \label{fig:pipeline}
% \end{figure}

% \begin{myitemize}
%     \item \textbf{View Specification} The view specification stage lets users define the input view (i.e., query) they want through a spreadsheet-style interface. The view is used to identify relevant datasets, which are those with attribute names or example tuples that appear in the input view. 
%     % The view specification stage lets users define a view they want. Through a spreadsheet-style interface, users can specify attribute names, a set of examples and data types to define the desired view. After that, the view specification stage will find all relevant columns for each attribute based on a clustering algorithm.\notera{this describes what it does, it also needs to say what challenge solves}
%     \item \textbf{View Search} The view search stage is responsible for finding join graphs and generating result views. To speed up the view search process, DoD incrementally materializes join paths by prioritizing higher-quality ones.
%     % After the view specification stage, we get candidate columns and tables for each attribute. Then, the view search stage is responsible for finding join paths between candidate tables, \notera{why does it have to incrementally materialize them?}incrementally materializing join paths and generating result views. \notera{as above, what challenges does this stage solve?}
%     \item \textbf{View Presentation} To navigate users to their preferred view among a pool of result views, we design a new method, \textit{4C} that reduces the size of the view choice space, and a presentation framework that guides users to find their preferred view by strategically asking them to answer automatically generated questions in an interactive way. 
%     % We designed a new method, \textit{4C}, which reduces the size of the view choice space by classifying the result views into four categories: \textit{compatible}, \textit{contained}, \textit{complementary} and \textit{contradictory}. Once the views are classified into the 4 groups, a view presentation framework will \notera{how does the guidance look like?}guide the users to find their desired view among the reduced view choice space. \notera{what problem does this stage solve?}
% \end{myitemize}


\subsection{Discovery Engine}
We use Aurum \cite{aurum}, an open-source data discovery platform as our discovery engine. Aurum reads relations from data sources such as databases, lakes, and files in filesystems, and produces a discovery index. The discovery index is logically a hypergraph where the nodes correspond to columns and edges represent relationships (content similarity or inclusion dependency) between columns. Based on this hypergraph, Aurum provides useful discovery APIs that can help upstream applications query the data. Next, we will introduce three Aurum APIs that will be used in our implementation.

\mypar{search\_content(\textit{keyword})} search the full-text-search index and return all columns that contain the input keyword. 

\mypar{content\_similar\_to(\textit{col})} Users can configure a similarity metric (e.g. overlap similarity) and a threshold in Aurum. In the process of building the discovery index, columns that have a similarity larger than the threshold will be connected. This API returns all columns that are similar to the input column w.r.t the pre-configured similarity metric.

\mypar{paths(\textit{table1}, \textit{table2}, \textit{max\_hop})} query the discovery index and retrieve all join paths between table1 and table2 w.r.t the maximum number of hops.


%The discovery index is logically a hypergraph where the nodes correspond to columns and edges represent relationships (e.g.inclusion dependency) between columns. Based on this hypergraph, Aurum provides an API to query join paths between two tables. Additionally, the discovery index also includes a full text search index of textual columns and their attribute names. Based on the full text search index, Aurum provides an API to query relevant columns that contain certain values.

\subsection{Column Selection}
In the column selection stage, users are given a spreadsheet-style interface where they can specify a set of examples for each attribute they want. When defining a view, users are trying to indicate DoD what datasets and columns are relevant. The crux of the column retrieval problem is to identify relevant columns based on user-given examples.

\textbf{Example 1} (Column Selection Strategy) Consider a user who wants to find columns representing COVID-19 vaccination facilities and provides the examples \{Walmart, Walgreens, UChicago Hospital\}. \dod first searches for columns matching each example using Aurum and lists results containing at least one example in \autoref{fig:example1}. \autoref{tab:columns} shows the information of each column including the table it belongs to, its name and the number of examples contained in it.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/example1.png}
  \caption{Tables that contain at least one user example}
  \label{fig:example1}
 \end{figure}

\begin{table}[h]
    \centering
     \begin{tabular}{||c c c c||} 
     \hline
     \# & table name & column name & \# Example \\ 
     \hline
     1 & covid19\_vaccine\_locations & facility & 2 \\ 
     \hline
     2 & flu\_vaccine\_locations & name & 3 \\
     \hline
     3 & pharmacy\_status & name & 2 \\
     \hline
     4 & chicago\_pharmacy\_2013 & name & 2 \\ 
     \hline
    \end{tabular}
    \caption{column information table}
    \label{tab:columns}
\end{table}

Many existing systems consider a column as relevant only if it contains all user-given examples(or contains the most number of examples) because \emph{they assume users have perfect knowledge}. Based on this strategy, only \textit{Column 2} will be selected in Example 1. However, this approach clearly misses the ground truth column, \textit{Column 1}. Normally, users do not exactly know what examples would yield the column of interest, and thus there tends to be noise in users' examples. Making decisions for users by only considering columns that contains all input examples could miss many relevant columns and hence missing right views. Additionally, tables in data lakes have many similar columns and semantic ambiguity, which further increase the difficulty of locating relevant columns for users.

Another approach adopted by many systems is to consider one column as relevant as long as it contains one input example. In this case, \textit{Column 1, 2, 3, 4} will all be selected. However, this approach tends to include many irrelevant columns like \textit{Column 3, 4} in the Example 1. In scenarios with many datasets, the number of columns that fulfill at least one example becomes large, leading to many join paths, lots of spurious views, and hence low performance.

% To find relevant datasets efficiently, DoD uses a clustering-based algorithm that clusters similar columns, reducing the space of options users need to consider and improving the possibility of finding relevant columns.

%In summary, our goal is to find as many relevant columns as possible and filter out irrelevant columns effectively. To achieve this goal, we propose a clustering-based algorithm. The major intuition is to cluster columns that have similar content and choose relevant columns based on clusters. 

\sg{To add for future: We choose this clustering algorithm because it is highly efficient.  Aurum gives nearest neighbors and this algorithm works well in practice. I can try to show tht this is similar to k-center algorithm.}

In summary, existing approaches either select too many columns which lead to poor system performance or select too few columns which could miss relevant columns. Additionally, no approaches let users check whether the system finds the right columns they want. Users can only see the generated views in the final presentation stage at which users can hardly tell which one is his/her desired view because there are too many similar views. However, directly presenting all columns that match at least one user example leaves users an impractical choice space. To tackle this problem, we propose a clustering-based algorithm. After grouping similar columns into clusters, we can reduce the space of options users need to consider and improve the possibility of finding relevant columns.

% \textbf{Similarity Metric} Users can configure similarity metric such as jaccard similarity or overlap similarity in Aurum. Aurum will build an index for the similarity metric in the pre-processing stage and DoD can query the nearest neighbors of one particular column efficiently through calling Aurum API \textit{content\_similar\_to()}. In the setting of DoD where tables are of various sizes, overlap similarity can better capture the similarity between different columns because jaccard similarity suffers from unbalanced sizes of columns.

\textbf{Clustering-based Column Retrieval} In the clustering-based column retrieval approach, we cluster similar columns because similar columns are likely to refer to the same entity. In other words, we not only select relevant columns based on example matching number but also consider columns that match less examples but refer to the same entity. Retrieving columns based on clusters can select more columns that are potentially relevant and thus be more noise-tolerant and robust. The clustering-based column retrieval approach is described in \autoref{algo_column_retrieval}. The first step is to find all columns that contain at least one example (line2-5). Then, we will cluster these candidate columns based on the similarity metric provided by Aurum as described in \autoref{algo_cluster}(line6). For each matching column, DoD finds its nearest neighbors based on Aurum API \textit{content\_similar\_to} (line 10) and then add the matching column and its neighbor columns to one cluster. Additionally, If two clusters intersect, DoD merges them into one cluster, improving recall (line 13, 16). After getting all clusters, each cluster will be assigned a score as described in \autoref{algo_score}(line7). The score of one cluster is the maximum number of examples contained in any column in that cluster. Finally, we select clusters that have the maximum score and all columns in them will be considered as relevant. (line 8-12)

In Example 1, the final content-based clusters are \{\textit{Column 1, 2}\}, \{\textit{Column 3, 4}\}. The score of each cluster is 3, 2 correspondingly. 

Our column retrieval stage supports both \textit{automatic mode} and \textit{human-in-the-loop mode}. 

In the \textit{automatic mode}, clusters with the highest score are selected and all columns in these clusters will be considered as relevant.

In the \textit{human-in-the-loop mode},  users have access to the clusters and can choose a different one if they know which is correct. But when they do not know which one is correct, the clustering-method helps steer the search process. Looking at clusters help users gain better knowledge of the data (e.g. concrete attributes they want, more accurate samples).

\IncMargin{1em}

\begin{algorithm}\SetKwFunction{Union}{Union} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$examples$: a list of examples of one column} 
	\Output{$candidate\_cols$: candidate columns relevant to $examples$}
	 \BlankLine 
	 
	 candidate\_cols $\leftarrow$ list[]
	 
	 \tcp*[h]{all columns containing at least one example}
	 
	 all\_cols $\leftarrow$ list[]
	 
	 \For{example $\in$ examples}
	 {
	    \tcp*[h]{get all columns containing the example}
	    
	    cols $\leftarrow$ aurum\_api.search\_content(example)
	    
	 	UNION(all\_cols, cols)
	 }
	 
	 clusters $\leftarrow$ cluster\_similar\_columns(all\_cols)
	 
	 cluster\_score $\leftarrow$ assign\_cluster\_score(clusters)
	 
	 max\_score = max(cluster\_score.values())
	 
	\For{cluster, score in cluster\_score}{
	    \If(){score == max\_score}{
	        candidate\_cols.merge(cluster)
	    }
	}
	 
	 \Return candidate\_cols
 	 	  \caption{Column Retrieval}
 	 	  \label{algo_column_retrieval} 
 	 \end{algorithm}
 \DecMargin{1em} 

\IncMargin{1em}

\begin{algorithm} \SetKwFunction{Union}{Union} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$cols$: a set of candidate columns} 
	\Output{$clusters$: Column Clusters}
	 \BlankLine 
	 
	 clusters $\leftarrow$ list[list[]]
	 
	 column\_cluster $\leftarrow$ map()
	 
	 idx $\leftarrow$ 0 
	 
	 \ForEach{col in cols}
	 {
	    \If()
	 		{col in column\_clusters}{ 
	 		\tcp*[h]{has been assigned a cluster}
	 		
	 		continue
	 		}
	 	cluster $\leftarrow$ set()
	 	
	 	cluster.add(col)
	 	
	 	cluster\_id $\leftarrow$ idx
	 	
	 	neighbors $\leftarrow$ aurum\_api.content\_similar\_to(col)
	 	
	 	\ForEach{neighbor in neighbors}{
	 	    \If(){neighbor in column\_cluster}{
	 	        \tcp*[h]{merge into the existing cluster}
	 	        
	 	        cluster\_id $\leftarrow$ column\_cluster[neighbor]
	 	    }
	 	    cluster.add(neighbor)
	 	}
	 	
	 	\ForEach{column in cluster}{
	 	    column\_cluster[column] $\leftarrow$ cluster\_id
	 	}
	 	
	 	idx $\leftarrow$ idx + 1
	 }
	 \tcp*[h]{construct clusters}
	 
	 \For{(column, cluster\_id) in column\_cluster}{
	    clusters[cluster\_id] = column
	 }
	 
	 \Return clusters
 	 	  \caption{Cluster Similar Columns}
 	 	  \label{algo_cluster} 
 	 \end{algorithm}
 \DecMargin{1em} 
 
 
 \IncMargin{1em}
 \begin{algorithm} \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up} \SetKwFunction{Union}{Union}\SetKwFunction{ContentSimilarTo}{ContentSimilarTo} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$clusters$: Columns clusters} 
	\Output{$cluster\_score$: a map between cluster and its score}
	 \BlankLine 
	 cluster\_score $\leftarrow$ map()
	 
	  \ForEach{cluster in clusters}
	 {
	    max\_example\_num $\leftarrow$ 0
	    
	    \ForEach{column in cluster}{
	    
	        example\_num $\leftarrow$ the number of examples contained in the column
	        
	        \If(){example\_num > max\_example\_num}{
	            max\_example\_num += 1
	        }
	    }
	    cluster\_score[cluster] $\leftarrow$ max\_example\_num
	 }
	 
	 \Return cluster\_score
        \caption{Assign Cluster Score}
 	 	  \label{algo_score} 
\end{algorithm}
 \DecMargin{1em} 


\subsection{Join Graph Search and Materialize}
\yg{todo: paraphrase the texts from arxiv paper}
\yg{todo: add pesudocode for explore join graphs}
% \notera{We need one paragraph that gives a top-bottom explanation of view search. It should provide a high-level idea of what are the different stages and why they are there. Then, we can go into the details of each of those -- as the text does now} \yg{Resolved}

In this component, we want to combine relevant columns obtained in the Column Retrieval stage. To achieve this goal, we organize the Join Graph Search and Materialize stage into four steps as described in \autoref{algo_view_search}. First, find all groups of tables that include as many user-wanted columns as possible (line 2). Second, check if a group of tables fulfilling a user's requirement is joinable or not. If it is joinable, explore all possible join graphs between tables (line 3-5). Thirdly, since we decide join graphs based on approximate inclusion dependency and content similarity, join graphs that we have explored in step 3 have various qualities. Thus, we need to sort them based on a scoring model and prioritize materializing "high-quality" ones (line 6). Last, materialize join graphs and produce candidate views (line 7). 

\subsubsection{\textbf{Find Candidate Groups}} A candidate group is a group of columns that covers as many attributes in the input view as possible. Each column is represented by a tuple (table, column\_name). Thus, each candidate group consists of two parts: a set of tables that covers users' input attributes and a set of columns indicating which column to project in the table after materializing the view. As described in \autoref{find_candidate_groups}, we first get all combinations of candidate columns obtained in the Column Retrieval stage (line 2). Then we iterate every combination to get its corresponding tables and columns (line 5-7). A set of tables and a set of columns can uniquely decide a candidate group. Note that a candidate group cannot be identified only by a set of tables because the columns to be projected could be different.

\subsubsection{\textbf{Explore Join Graphs}} After getting all candidate groups, the next step is to select joinable group and explore join graphs among them. A joinable group is a candidate group in which all the tables contained can be combined into one single table through the relational join operation. There may be multiple ways of joining the tables of a joinable group. This can happen if there exists more than one inclusion dependency between a pair of tables, or there are different intermediate tables that can be used to join two tables. Each strategy to join such tables is called a join graph. A joinable group, then, is a candidate group for which there is at least one existing join graph.

For each candidate group, DoD must find all join graphs that permit combining all tables. It is necessary to find all join graphs because some may be using a wrong inclusion dependency (leading to a wrong view) or one that is correct, but incompatible with the user’s intent—when there are different semantic views that fulfill the query view. To find all the join graphs, DoD first finds all the join paths between every pair of tables in the group. Then, it combines join paths together to form join graphs that permit joining all tables in the group. DoD discards duplicate join graphs—those that join the same tables on the same attributes—as well as join graphs that do not join every table in the group.

In order to identify a join path between a pair of tables, DoD uses Aurum API \textit{paths(table1, table2, max\_hop)}, which returns all join paths between two tables given a maximum number of hops, by querying its discovery index.

\subsubsection{\textbf{Sort Join Graphs}}
Since we are using approximate inclusion dependency instead of strict PK/FK relationship, some generated join paths will use wrong attributes, or will lead to semantically different views. Because evaluating a join graph is expensive, materializing all join graphs at once without any ranking strategy on a large dataset can take a few minutes, leading to poor user experience. Hence, we devise a scoring model that prioritizes materializing "high-quality" join graphs.

A "high-quality" join graph is defined as having "high-quality" join operations and involves less number of tables. "high-quality" join operation means join performed on keys that are more likely to be PK/FK. To measure this property, we calculate and store the uniqueness score \footnote{$uniqueness\_score(column) = \frac{len(set(column))}{len(column)}$} of each column. For a join operation on column a and b, the score of this join is defined as the maximum uniqueness score between a and b. The final scoring formula considers both the quality of each join and the number of joins.
\begin{equation}\nonumber
    % Score(jp) = \frac{\sum_{join \in jp} score(join)}{COUNT(join)} - \sigma (Count(join) - 2)
    Score(join\_graph) = \frac{avg(score(join \in join\_graph))}{1 + ln(1+ln(\#tables))}
\end{equation}

DoD sorts all join graphs based on this scoring model and passes them to the materialization stage. Then, join graphs of "high-quality" and that are easy to compute will be materialized and presented to users first.

\subsubsection{\textbf{Materialize a Join Graph}}
A join graph contains the information necessary to join a set of N tables. The join graph nodes represent the tables, and an edge between two nodes indicates that the two tables can be joined together. Each node contains the attribute on which the table should be joined.

To materialize a join graph, joins are performed from the leaf nodes to inner ones. A leaf node is one that is connected to only another one. Every time a join is performed, its node and edge are removed. The procedure repeats N-1 times, until the resulting joined table is obtained.

% \textbf{Join Path Exploration} Each subset of candidate tables that contain all attributes in the input view is called a \textit{candidate group}. For each \textit{candidate group}, DoD identifies all possible join paths that combine the tables in the candidate group into the resulting view. DoD uses Aurum's derived \textit{approximate} inclusion dependencies. An approximate inclusion dependency between two columns exists when values of one column are approximately included in the other. This helps with two practical problems. First, it is sometimes useful to use approximate keys to combine datasets that would not be able to be combined otherwise. This is true when tables come from different sources and nobody assigned a PKFK at the design time. Second, because data is dirty, if we only considered exact keys, we would ignore opportunities to combine datasets. To find a join path, we first find all the join paths between every pair of tables in the group using the discovery API of Aurum \cite{aurum}; then, combine the join paths together to form a single \emph{join graph}.

\begin{algorithm} \SetKwFunction{AllCombinationOf}{AllCombinationOf} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$attribute\_candidates$: each attribute in the view and its corresponding candidate columns,\\
	$offset$: the expected number of output pj-views
	} 

	\Output{$pj\_views$: list of candidate pj-views}
	\BlankLine
	all\_join\_graphs $\leftarrow$ list[]
	
	G $\leftarrow$ find\_candidate\_groups(attribute\_candidates)
	 
	 \ForEach{candidate\_group in G}
	 {
	    join\_graphs $\leftarrow$ explore\_join\_graphs(candidate\_group)
	    
	    all\_join\_graphs.append(join\_graphs)
	 }
	 
	 sorted\_graphs $\leftarrow$ sort\_join\_graphs(all\_join\_graphs)
	 
	 pj\_views $\leftarrow$ materialize\_views(sorted\_graphs[0:offset])
	
	\Return pj\_views
    \caption{Join Graph Search and Materialize}
 	\label{algo_view_search} 
\end{algorithm}

\begin{algorithm} \SetKwFunction{AllCombinationOf}{AllCombinationOf} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$attribute\_candidates$: each attribute in the view and its corresponding candidate columns} 
	\Output{$G$: a list of candidate groups}
	 \BlankLine 
	 G $\leftarrow$ list()
	 
	  \ForEach{group in \AllCombinationOf(attribute\_candidates)}
	 {
	    candidate\_group\_table $\leftarrow$ set()
	    
	    candidate\_group\_column $\leftarrow$ set() 
	    
	    \ForEach{column in group}{
	    
	       candidate\_group\_table.append(column[table])
	       
	       candidate\_group\_column.append(column)
	       
	    }
	    
	    candidate\_group $\leftarrow$ (candidate\_group\_table, candidate\_group\_column)
	    
	    G.append(candidate\_group)
	 }
	  \Return G
        \caption{Find Candidate Groups}
 	 	  \label{find_candidate_groups} 
\end{algorithm}

\begin{algorithm} \SetKwFunction{AllCombinationOf}{AllCombinationOf} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	
	\Input{$candidate\_group$: a candidate group consisting of relevant tables \\
	$max\_hop$: maximum join hops between every pair of tables} 

	\Output{$join\_graphs$: join graphs to combine tables in the $candidate\_group$}
	\BlankLine
	all\_join\_graphs $\leftarrow$ list[]
	
	G $\leftarrow$ find\_candidate\_groups(attribute\_candidates)
	 
	 \ForEach{candidate\_group in G}
	 {
	    join\_graphs $\leftarrow$ explore\_join\_graphs(candidate\_group)
	    
	    all\_join\_graphs.append(join\_graphs)
	 }
	 
	 sorted\_graphs $\leftarrow$ sort\_join\_graphs(all\_join\_graphs)
	 
	 pj\_views $\leftarrow$ materialize\_views(sorted\_graphs[0:offset])
	
	\Return pj\_views
    \caption{Explore Join Graphs}
 	\label{algo_explore_graphs} 
\end{algorithm}

\subsection{View Presentation}

\notera{we likely want to explain 4C first to conceptualize the mental mdoel we have to think of views that come from the same input definition. Then we can use 4C as part of the presentation framework}
\zz{yes we need formal definitions of the 4 groups (along with the candidate key), how it's suitable for the data lake setting, and then explain how it's incorporated into the presentation framework.}
\notera{can you add the formal definitions? you can start with what's in the dod-arxiv paper and improve on that.}

\notera{the algos could have the same formatting as those in the previous sections}

\notera{give a top-bottom explanation of view presentation. First, what's its goal. Second, how is that goal achieved, what are the components of the solution. Last, explain in detail the components of the solutions---here's where the algorithms may help a lot}

Given a set of output views, the goal of view presentation stage is to reduce the view choice space and help users and software identify their preferred view by presenting the results in an informative way. Although we can prioritize which joins paths to materialize, users may still be left with a large view choice space, given that the number of candidate tables or potential join paths can be extremely large. Moreover, the output views can contain may contain many noises or conflicting information due to incorrect join paths that makes it difficult for users \zz{and software?} to identify their preferred view. We introduce the two major components of view presentation stage to address these two challenges:

\zz{come up with a different name? This component can be used alone (for the automatic mode)}
\subsubsection{\textbf{4c method}} \zz{explain the motivation behind 4c: 1. reduces the size of view choice space 2. generates signals that can be used as questions during human-in-the loop mode} In order to reduce the size of view choice space, we designed a novel method, called \textit{4C}, that classifies the output views into four categories: \textit{Compatible}, which means that views are identical; \textit{Contained}, which means that the values of one view subsume others; \textit{Complementary}, which means that the set difference of tuples of views is not empty; and \textit{Contradictory}, which means that certain tuples are incompatible across views. Whether a pair of view is \textit{complementary} or \textit{contradictory} depend upon the candidate key it's comparing to. More formally:

\begin{definition}[Output view]
An output view, $v_i$, contains a set of rows, $R_i$, that can be retrieved with the function $f$, $f(v_i) = R_i$. 
\end{definition}

\begin{definition}[Candidate key]
\zz{?they might not be 100\% unique if we limit the candidate key size} A candidate key, $k$, is a set of attributes in an output view, $v_i$, that can uniquely identify each row in $R_i$. We can refer to a row, $r_i \in R_i$, with its candidate key value, $k_i$, which we can use to obtain the row; $k(R_i, k_i) = r_i$. There can be multiple candidate keys in $v_i$ that satisfy this property. 
\end{definition}

\begin{definition}[Compatible views]
Two candidate views, $v_1$ and $v_2$, are compatible if they have the same cardinality $|R1| = |R2|$, and their set of tuples is exactly the same: $|(R_1 \setminus R_2)| = 0$ and $|(R_2 \setminus R_1)| = 0$, where the symbol $\setminus$ indicates the set difference operation.
\end{definition}

\begin{definition}[Contained views]
A view, $v_1$, contains another view, $v_2$, when $|(R_1 \setminus R_2)| > 0$ and $|(R_2 \setminus R_1)| = 0$, that is, when all rows of $v_2$ are contained in $v_1$.
\end{definition}

\begin{definition}[Complementary views]
Two views, $v_1$ and $v_2$ are complementary if the two views have the same candidate key, $k$, and $|(K_1 \setminus K_2)| > 0$ and $|(K_2 \setminus K_1)| > 0$, where $K_1$ and $K_2$ are the set of candidate key values for $v_1$ and $v_2$ respectively. That is, each view has candidate key values not contained in the other view.
% Two views, $v_1$ and $v_2$ are complementary when $|(R_1 \setminus R_2)| > 0$ and $|(R_2 \setminus R_1)| > 0$, that is, each view has rows not contained in the other view.
\end{definition}

\begin{definition}[Contradictory views]
Two views, $v_1$ and $v_2$ are contradictory if the two views have the same candidate key, $k$, and a key value that exists in both views, $k_i \in K_1, K_2$, yields distinct rows, $k(R_1; k_i) \neq k(R_2; k_i)$. Two rows are distinct when any value of any of their attributes is different.
\end{definition}

Note that although the description above refers to two views, the 4C method classifies multiple views into each of the above categories. For example, a view can be compatible with other views, contains other views, and be complementary or contradictory to other views on a candidate key, all at the same time.
% For example, many views can be compatible among themselves. One view may contain many other views. One single view can be complementary with respect to many others, and contradict many others as well. Similarly, a view can contain another view, be complementary to another one, compatible with another group and be in contradiction with other views on different rows, all at the same time. 
Next, we present the algorithm we use to classify the output views into the four above categories.

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$V$, collection of output views}
\KwOutput{$G$, views classified per class and schema type}
 \BlankLine
 $S \leftarrow classify\_per\_schema(V)$\; \label{4c_main:classify_per_schema}
 \For{$s \in S$}{ \label{4c_main:loop_schema}
    $C1 \leftarrow identify\_c1(V)$\; \label{4c_main:c1}
    $SC1 \leftarrow select\_representative\_c1(C1)$\; \label{4c_main:select_representative_c1}
    $C2, C34 \leftarrow identify\_c2\_and\_candidate\_c3c4(SC1)$\; \label{4c_main:c2} 
    $C3, C4 \leftarrow identify\_c3\_and\_c4(candidate\_C3C4)$\; \label{4c_main:c3_c4} 
    $G[s] \leftarrow (C1, C2, C3, C4)$\;
 }
 \Return $G$\;
 \caption{Main 4C}
 \label{4c_main}
\end{algorithm}

The main body of the algorithm is shown in \autoref{4c_main}. Because 4C works on views with the same schema (attributes in this case), the first step is to separate the output views into groups according to their schema (\autoref{4c_main:classify_per_schema}). Then, the algorithm runs the 4C classification for each group (\autoref{4c_main:loop_schema}), leading to the classification of views into the four categories: \textit{compatible} ($C1$), \textit{contained} ($C2$), \textit{complementary} ($C3$), and \textit{contradictory} ($C4$). It will first identify quickly the compatible and contained views. Then, it identifies complementary and contradictory views among the remaining ones.

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$V$, collection of output views}
\KwOutput{$C1$, collection of lists, each list contains $v \in V$ that are compatible}
 \BlankLine
 $g \leftarrow map()$\;
 \For{$v_i \in V$}{
    $hv_i \leftarrow hash(v_i)$\; \label{4c_compatible:hash}
    $add(g, hv_i, v_i)$\;
 }
 $C1 \leftarrow g.values()$\;
 \Return $C1$\;
 \caption{identify\_c1}
 \label{4c_compatible}
\end{algorithm}

\mypar{Identify compatible views} \zz{copied from dod paper} The next step is to identify groups of views that are compatible ($C1$) with each other. The main idea is to hash each view (\autoref{4c_compatible:hash}), and insert the view on a map that is keyed on the hash value. A view hash is the sum of its rows hashes, and a row hash is the sum of its cells hashes. With this hashing method, compatible views are guaranteed to have the same hash value, so this is an efficient way of identifying groups of compatible views fast.

Because all compatible views are identical, in the Main 4C algorithm, we select one only to continue the classification (\autoref{4c_main:select_representative_c1}). The selected views are then given to a function in charge of identifying contained groups ($C2$), as well as groups that may be either complementary or contradictory ($C34$), see \autoref{4c_main:c2}.

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$SC1$, collection of output views}
\KwOutput{$C2$, list of tuples $(v_C, [vc])$; $v_C$ contains all $[v_c]$. $C34$, list of tuples $(v_i, v_j, I_i, I_j )$; $I_{i,j}$ are the sets of row indices in which $v_i$ and $v_j$ disagree}
 \BlankLine
 $(gc2, gc34) \leftarrow (map(), map())$\;
 \For{$(v_i, v_j) \in pair(SC1)$}{ \label{4c_contained:loop}
    $(h\_list_i, h\_list_j) \leftarrow (hash\_rows(v_i), hash\_rows(v_j))$\;
    $(h\_set_i, h\_set_j) \leftarrow (set(h \_list_i), set(h\_list_j))$\;
    \eIf{$len(h\_set_i) \geq len(h \_set_j)$}
    { \label{4c_contained:if_start}
        \If{$(h\_set_j \setminus h\_set_i) = 0$}{
            $add(gc2, v_i, v_j)$\;
        }
    \label{4c_contained:if_end} }
    { \label{4c_contained:else_start}
        $s_{ij} \leftarrow h\_set_i \setminus h\_set_j$\;
        $s_{ji} \leftarrow h\_set_j \setminus h\_set_i$\;
        \If{$s_{ij} \geq 0 \land s_{ji} \geq 0$}{
            $I_i \leftarrow indices(h\_list_i, s_{ij})$\;
            $I_j \leftarrow indices(h\_list_j, s_{ji})$\;
            $add(gc34, v_i, v_j, I_i, I_j)$\;
        }
    } \label{4c_contained:else_end}
 }
 $(C2, C34) \leftarrow (unpack(gc2), unpack(gc34))$\;
 \Return $(C2, C34)$\;
 \caption{identify\_c2\_and\_candidate\_c3c4}
 \label{4c_contained}
\end{algorithm}

\mypar{Identify contained views} \zz{copied from dod paper} The function to finding contained views is shown in \autoref{4c_contained}. For each pair of views (\autoref{4c_contained:loop}), the algorithm obtains the list and the set of hashes of each view respectively. The list will be used to identify indexes of rows (because it maintains the order), while the sets are used to quickly tell whether the views are contained or may be complementary. \autoref{4c_contained:if_start}--\autoref{4c_contained:if_end} checks whether the hashes of one view are completely contained on the first, in which case the view is contained in the first and this is recorded in the variable $gc2$. Note that because the loop enumerates pairs of views in both directions, it is not necessary to check for containment in both directions here.

If the views are not contained, the algorithm tries to decide if they are candidates for the complementary and contradictory group. This decision is done in \autoref{4c_contained:else_start}--\autoref{4c_contained:else_end}. The algorithm computes the set difference of rows in both directions and checks whether it is non-empty in both cases. When it is, this indicates that each view has hashes not contained in the other view. This can be caused for two different reasons: either one view has rows that are non existent in the other (a case of complementarity), or the values of certain rows differ in some values, which would also lead to different hashes and indicate a contradiction. The algorithm returns the identified groups of contained views as well as those that may be complementary or contradictory.

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$C34$, list of tuples $(v_i, v_j, I_i, I_j)$; $I_{i,j}$ are the sets of row indices in which $v_i$ and $v_j$ disagree}
\KwOutput{$C3$, list of tuples $(v_i, v_j, k, K_i, K_j)$, $K_{i,j}$ are the sets of key values of candidate key $k$ in $v_i$ and $v_j$ that are complementary. $C4$, list of tuples $(v_i, v_j, k, K)$, $K$ is the set of key values of candidate key $k$ in which $v_i$ presents a contradiction with respect to $v_j$}
 \BlankLine
 $(C3;C4) \leftarrow (set(), set())$\;
 \For{$(v_i, v_j, I_i, I_j) \in C34$}{ \label{4c_contra_compl:loop}
    $vsel_i \leftarrow select(v_i, I_i)$\; \label{4c_contra_compl:select_i}
    $vsel_j \leftarrow select(v_j, I_j)$\; \label{4c_contra_compl:select_j}
    $k\_list \leftarrow find\_candidate\_keys(v_i, v_j)$\; \label{4c_contra_compl:find_keys}
    \For{$k \in k\_list$}{ \label{4c_contra_compl:for_key}
        $KV_i \leftarrow project(vsel_i, k)$\; \label{4c_contra_compl:project_i}
        $KV_j \leftarrow project(vsel_j, k)$\; \label{4c_contra_compl:project_j}
        $K\_intersect \leftarrow KV_i \cap KV_j$\; \label{4c_contra_compl:k_intersect}
        $K \leftarrow find\_contr(vsel_i, vsel_j, K\_intersect)$\; \label{4c_contra_compl:find_contr}
        $add(C4, v_i, v_j, k, K)$\;
        \If{$len(K) = 0$}{
            $K\_compl \leftarrow (KV_i \cup KV_j ) \setminus K\_intersect$\;  \label{4c_contra_compl:k_compl}
            $(K_i, K_j) \leftarrow find\_compl(vsel_i, vsel_j, K\_compl)$\; \label{4c_contra_compl:find_compl}
            $add(C3, v_i, v_j, k, K_i, K_j)$\;
        }
    }
 }
 \Return $(C3, C4)$\;
 \caption{identify\_c3\_and\_c4}
 \label{4c_contra_compl}
\end{algorithm}

\mypar{Identify complementary and contradictory views} The last part of the algorithm is to identify which pairs of views in C34 are complementary and which are contradictory. This corresponds to \autoref{4c_main:c3_c4} in the main body of \autoref{4c_main}. The body of this function is shown in more detail in \autoref{4c_contra_compl}. For each pair of views (\autoref{4c_contra_compl:loop}), it checks whether the different values (hashes) identified between this pair are due to complementarity or contradictions. For that, it first selects the relevant rows from each view (\autoref{4c_contra_compl:select_i}--\autoref{4c_contra_compl:select_j}) and obtains all possible candidate keys, $k\_list$ of the two views (\autoref{4c_contra_compl:find_keys}. Then for each candidate key (\autoref{4c_contra_compl:for_key}), it projects the attributes of that key into the selection (\autoref{4c_contra_compl:project_i}--\autoref{4c_contra_compl:project_j}). This
produces $KV_i$ and $KV_j$ , which are the sets of key values that correspond to the distinct hashes of each view. At this point, the intersection of these two sets, $K\_intersect$, corresponds to the contradictory examples (\autoref{4c_contra_compl:k_intersect}--\autoref{4c_contra_compl:find_contr}), while the rest of values, $K\_compl$, correspond to the complementary ones (\autoref{4c_contra_compl:k_compl}--\autoref{4c_contra_compl:find_compl}). \zz{this is just based on the current implementation} Two views are only complementary if no contradictions exist. Therefore, each candidate key of a pair of views corresponds either contradictory or complementary relationship.

\smallskip
Once finished, all views will be classified into the four categories. By applying the \textit{4C} method, we are able to prune a portion of the output views; e.g. we can discard \textit{compatible} views, leaving only one view in each group, and choose the view with the highest cardinality among each group of \textit{contained} views \zz{since ... (need reasons)}. The user still has to choose among the rest of the views. The most naive approach would be letting the user look through all the rest of views and choose their preferred one, but this approach can be very ineffective and tedious for the user since the amount of views left may still be very large and and views can be noisy and spurious. To leverage the \textit{complementary} or \textit{contradictory} relationships we obtained using the \textit{4C} method, we designed a \textit{human-in-the-loop} presentation framework that reduces user's effort and guide them towards their preferred view with minimal amount of interactions by asking them questions strategically.

\zz{Add applying S4 ranking to the views here, so we can use the ranking alone without proceeding to the next step. But don't know how to make the transition.}
\zz{maybe instead mention S4 ranking in evaluation?}

\subsubsection{\textbf{Human-in-the-loop}}
We now introduce the human-in-the-loop presentation framework. Intuitively, we can present each pair of complementary or contradictory views with their corresponding candidate keys at each interaction; to help user distinguish between the two views, we can present only the complementary or contradictory rows to highlight the differences between the two views. At every interaction, the user selects between each pair of views, pruning out the view they don't like, and ultimately finds the view they want either by going through every pair until there is no more pair left to present, or stopping early since they already found their preferred view among the views that have been shown to them. 

However, this method has two limitations: (1) the number of complementary or contradictory view pairs can be enormous, and the user has to go through all the pairs to explore all views at least once; in the worst case, if all output views are either complementary or contradictory to each other, the number of view pairs to present grows exponentially based on the total number of views. (2) since the user may only have limited domain knowledge and they can be uncertain of which view is the exact one they want, they may need more interactions to explore more views and build up confidence as of the views they choose. Thus pruning out views directly can potentially discard views users actually want. \zz{second point needs rephrasing -- just trying to show why we need a scoring model}

To tackle theses two limitations, we designed an \textit{uncertainty framework} \zz{better name?} that is able to (1) let user's selections influence more than just a pair of views at each interaction, thus reducing the number of interactions they would need to explore all the views \zz{very subtle here. Although we still have exponential number of pairs, we don't have to go through all of them in order to explore all views. how to phrase it more nicely?}, and (2) assign scores to each view and re-rank them at each interaction instead of pruning out views directly, so user can make a more informed decision of which view they prefer based on the view scores. And most importantly, the \textit{uncertainty framework} presents questions strategically, in a way that reduces\zz{? maybe not use the word minimize without clear definition} the number of interactions user needed in order to find their preferred view.

We now formally define the \textit{complementary set} and \textit{contradictory set} that we designed to address the first point from above.

\begin{definition}[Complementary set]
\zz{?}
Two sets of views, $s_1 \subseteq V$ and $s_2 \subseteq V$, form a \textit{complementary set}, if they all share the same candidate key, $K$, and there exists two key values, $k_i \in K_i$ and $k_j \in K_j$ where $k_i \neq k_j$, such that for all the views $v_i \in s_1$, the row $r_1 = k(R_i, k_i)$ is the same; for all the views $v_j \in s_2$, the row $r_2 = k(R_j; k_j)$ is the same. Finally, $k_i \notin K_j, k_j \notin K_i$. That is, $r_1$ and $r_2$ is complementary with each other, and $r_1$ is not contained in any of the views in $s_2$, $r_2$ is not contained in any of the views in $s_1$.
\end{definition}

\begin{definition}[Contradictory set]
\zz{?}
Two sets of views, $s_1 \subseteq V$ and $s_2 \subseteq V$, form a \textit{contradictory set}, if they all share the same candidate key, $K$, and there exists a key value, $k$, such that for all the views $v_i \in s_1$, the row $r_1 = k(R_i; k)$ is the same; for all the views $v_j \in s_2$, the row $r_2 = k(R_j; k)$ is the same. Finally, $r_1 \neq r_2$, meaning $r_1$ and $r_2$ is contradictory on the key value $k$, which is present in all the views in both $s_1$ and $s_2$.
\end{definition}

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$M$, double-nested map where the first key is the view pair $(v_i, v_j)$ that exist in $C3$ or $C4$, and the second key is its candidate key $k$, the corresponding value is either $(K_i, K_j)$, meaning it is complementary, or $K$, meaning it is contradictory. $sample\_size$, maximum number of contradictory or complementary rows in a signal}
\KwOutput{$(S\_compl, S\_contra)$, lists of complementary and contradictory signals consisting of tuple $(k, S_1, S_2, R_1, R_2)$.}
 \BlankLine
 \ForEach{$(v_i, v_j)$ in $M$}{
    \ForEach{$k$ in $M[(v_i, v_j)]$}{
        $(S_1,  S_2) \leftarrow (set(), set())$\;
        $(R_1,  R_2) \leftarrow (set(), set())$\;
        \eIf{$is\_compl(M[(v_i, v_j)][k])$}{
            $(K_i, K_j) \leftarrow M[(v_i, v_j)][k]$\;
            $(SK_i, SK_j) \leftarrow sample(K_i, K_j, sample\_size)$\; \label{generate_signals:sample_compl}
            \For{$(k_i, k_j) \in (SK_i, SK_j)$}{
                $r_1 \leftarrow k(R_i, k_i)$\;
                $r_2 \leftarrow k(R_j, k_j)$\;
                $(s_1, s_2) \leftarrow get\_compl\_set(r_1, r_2)$\; \label{generate_signals:get_compl_set}
                $add(S_1, s_1)$\; \label{generate_signals:combine_compl_start}
                $add(S_2, s_2)$\;
                $add(R_1, r_1)$\;
                $add(R_2, r_2)$\; \label{generate_signals:combine_compl_end}
            }
            $add(S\_compl, k, S_1, S_2, R_1, R_2)$\;
        }
        {
            $K \leftarrow M[(v_i, v_j)][k]$\;
            $SK \leftarrow sample(K, sample\_size)$\; \label{generate_signals:sample_contra}
            \For{$k_i \in SK$}{
                $r_1 \leftarrow k(R_i, k_i)$\;
                $r_2 \leftarrow k(R_j, k_i)$\;
                $(s_1, s_2) \leftarrow get\_contra\_set(r_1, r_2)$\; \label{generate_signals:get_contr_set}
                $add(S_1, s_1)$\; \label{generate_signals:combine_contra_start}
                $add(S_2, s_2)$\;
                $add(R_1, r_1)$\;
                $add(R_2, r_2)$\;\label{generate_signals:combine_contra_end}
            }
            $add(S\_contra, k, S_1, S_2, R_1, R_2)$\;
        }
    }
 }
 \Return $(S\_compl, S\_contra)$\;
 \caption{generate\_signals}
 \label{generate_signals}
\end{algorithm}

For each pair of view, we can then generate \textit{complementary signals} and \textit{contradictory signals} to present through the procedure in \autoref{generate_signals}. \zz{I tried to properly define the signal but don't know how to, instead I just explained it through the algorithm. May still need to define it} Depending on the candidate key of each pair of view, we sample certain number of complementary or contradictory rows (\autoref{generate_signals:sample_compl} and \autoref{generate_signals:sample_contra}), and obtain the corresponding complementary or contradictory set for each sampled row (\autoref{generate_signals:get_compl_set} and \autoref{generate_signals:get_contr_set}). We then combine them together so that each signal contains multiple rows along with the combined complementary or contradictory set (\autoref{generate_signals:combine_compl_start}--\autoref{generate_signals:combine_compl_end} and \autoref{generate_signals:combine_contra_start}--\autoref{generate_signals:combine_contra_end}). 

\zz{may need to restructure this paragraph}
By changing from presenting complementary or contradictory view pairs to complementary or contradictory signals, we allow the user to explore multiple views by examining only a few pair of complementary or contradictory rows. At each interaction, the presentation framework presents a signal, which consists of the candidate key, $k$, two sets of complementary or contradictory rows, $R_1$ and $R_2$, that correspond to $k$, and their respective combined complementary or contradictory set, $S_1$ and $S_2$. Thus the signal presents two options, $R_1$ and $R_2$. The user chooses which set of rows they prefer; depending on their choice, the presentation framework increments the scores of views in the corresponding complementary or contradictory set. Optionally, the user can choose to select neither options, and in this case all views that are present in both sets will be decremented \zz{reason?}. In addition to updating view scores, the presentation framework also maintains a scoring model for all candidate keys across different signals. It increments the score of the current candidate key if the user selects an option since their action implies the candidate key and the complementary or contradictory values it yields are good enough for the user to make a decision; otherwise, if the user does not select any option, it decrements its score. The candidate key scores are used to determine the subset of signals the framework will consider; at each interaction, it will consider the signals with the candidate key that has the highest score. Choosing the best candidate key can help preventing presenting signals with schema (list of attributes) that the user prefer less, and instead present signals with associated complementary or contradictory relationships that the user agrees on.

\mypar{Uncertainty framework} One crucial aspect of the presentation framework is about picking which signal signal to present at each interaction. As our goal is to reduce user's effort of finding their preferred view, we should prioritize presenting signals that delivers more information about the output views and helps the user converge on the view they prefer the most in fewer amount of interactions. We first define the \textit{score threshold} and the \textit{information gain} of a signal as follows:

\begin{definition}[score threshold]
Given a percentile, $p$, the score threshold is the $p$-th percentile of the current scores of all views in the scoring model.
\end{definition}

\begin{definition}[Information gain of a signal]
The information gain of a signal describes the expected \textit{uncertainty removed}; that is, the expected number of views we are able to update with new information. Given a score threshold, $\tau$, we first obtain the new sets of views, $NS_1$ and $NS_2$, which are the subset of views in $S_1$ and $S_2$ of the signal with scores greater than $\tau$. Then, we quantify the information gain of a signal as :
\[ G = N - \sum_i p_i \cdot n_i \]
where $N$ is the total number of views in $NS_1$ and $NS_2$, $p_i$ is the probability of updating the views in $NS_i$ \zz{this is really just $n_i/N$}, and $n_i$ is the number of views in $NS_i$.
\end{definition}

\begin{algorithm}
\SetAlgoLined
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\KwInput{$V$, collection of output views. $sample\_size$, maximum number of contradictory or complementary rows in a signal. $p$, percentile for computing score threshold $\tau$.}
\KwOutput{$view\_scores$, list of tuples $(v_i, score_i)$, $v_i$ is the output view $v_i \in V$, and $score_i$ is the final score of $v_i$ of the last interaction}
 \BlankLine
 $G \leftarrow main\_4c(V)$\;
 \tcc{discard compatible views, leaving only one view in each group}
 $prune\_compatible\_views(G)$\;
 \tcc{keep the view with the highest cardinality among each group of contained views}
 $prune\_contained\_views(G)$\;
 \tcc{transform the pruned 4C views into the map $M$ which is the input to $generate\_signals$}
 $M \leftarrow transform(G)$\;
 $(S\_compl, S\_contra) \leftarrow generate\_signals(M, sample\_size)$\;
 $view\_scores \leftarrow initialize\_view\_scores()$\;
 $key\_scores \leftarrow initialize\_key\_scores()$\;
 \While{user continues interacting}{
    $k \leftarrow get\_best\_key(key\_scores)$\;
    $\tau \leftarrow compute\_threshold(view\_scores, p)$\;
    $signal \leftarrow pick\_next\_signal(S\_compl, S\_contra, k, \tau)$\;
    $(k, S_1, S_2, R_1, R_2) \leftarrow signal$\;
    \eIf{$is\_contradictory(signal)$}{
        $present\_complementary\_signal(k, S_1, S_2, R_1, R_2)$\;
        $pop(S\_compl, signal)$\;
    }
    {
        $present\_contradictory\_signal(k, S_1, S_2, R_1, R_2)$\;
        $pop(S\_contra, signal)$\;
    }
    $selection \leftarrow get\_user\_response()$\;
    \eIf{$selection \neq \emptyset$}{
        \tcc{increment the scores of views in the set that corresponds to user's selection}
        $increment\_view\_scores(view\_scores, selection)$\;
        $increment\_key\_scores(key\_scores, k)$\;
    }{
        \tcc{decrement the scores of all views in $S_1$ and $S_2$}
        $decrement\_view\_scores(view\_scores, S_1, S_2)$\;
        $decrement\_key\_scores(key\_scores, k)$\;
    }
 }
 \Return $view\_scores$\;
 \caption{View Presentation}
 \label{view_presentation}
\end{algorithm}

Consequently, at every interaction, the presentation framework computes the current score threshold, $\tau$, and picks the signal that has the highest information gain with respect to $\tau$ among the subset of signals with the candidate key that has the highest score. By considering views that have scores above the threshold when computing the information gain, the presentation framework is able to pick the most informative signal that allows the user to explore more views among the subset of views which they have a stronger preference on.

The overall algorithm of the presentation framework is outlined in \autoref{view_presentation} \zz{there isn't any need to go over the algorithm line by line?}. The interaction model continues until the user is satisfied with their selections and decides to settle with the current view scores. They may decide to pick the view with the highest score as their final view, or they can choose among the $top-k$ views. 

\smallskip

By dividing the end-to-end pipeline into three inter-connecting stages: view specification, view search and view presentation, DoD is able to navigate the user through different stages and find their preferred views efficiently and effectively. 

==> sections/view_spec_eval.tex <==
\subsection{View Specification Evaluation}

We want to answer the following key questions through the evaluation of view specification stage.
\begin{itemize}
    \item Does the view spec stage achieve the goal of finding relevant columns thoroughly and precisely?
    \item Does the view spec stage save user efforts?
    \item How does the view spec stage affect view search?
\end{itemize}

We evaluate and compare the following three algorithms.
\begin{itemize}
    \item \textbf{\textit{Select-All}} Choose all columns that contain at least one user example as relevant. \textit{Select-All} is equivalent to how S4 \cite{s4} decides relevant columns.
    \item \textbf{\textit{Select-Best}} Only consider columns that contain the most number of examples as relevant. \textit{Select-Best} is equivalent to how Squid \cite{squid} chooses relevant columns.
    \item \textbf{\textit{Select-Cluster}} First find all matching columns that contain at least one user example, then cluster them as described in Algorithm 1. Last, choose clusters that have the highest score.
\end{itemize}

\subsubsection*{\textbf{Q1: Does Select-Cluster find relevant columns thoroughly and precisely?}}

\subsubsection*{\textbf{Dataset and Groundtruth}} We use the dataset and ground truth from \cite{tableUnionSearch}. They collect 1405 tables from Canadian and UK Open Data and synthesize a ground truth indicating what columns are unionable. Unionable columns are columns that refer to the same entity. We adapt their ground truth through only keeping unionable columns that have overlap with each other because DoD only considers set similarity. \yg{TODO: Explain how i generate samples}

\subsubsection*{\textbf{DoD Setup}} The major parameters in \textit{Select-Cluster} are the similarity metric and similarity threshold. These two parameters can be configured in Aurum. In this section, we set the similarity metric as overlap similarity \footnote{overlap(A, B) = $\frac{|A \cup B|}{min(|A|, |B|)}$} and the similarity threshold as 0.8.

\subsubsection*{\textbf{Metric}}
\begin{itemize}
    \item \textbf{Recall} $\frac{TP}{TP + FN}$, measures how many correct columns you can find.
    Low recall will decrease the possibility for users to find their desired views.

    \item \textbf{Precision} $\frac{TP}{TP + FP}$, measures how many found columns are correct. Low precision will increase noise and overhead to the view search and presentation stage.

    \item \textbf{F1 score} $\frac{2*Precision*Recall}{Precision + Recall}$
\end{itemize}

The evaluation result on Open data is shown in \autoref{fig:q1}. Our \textit{Select-Cluster} method achieves higher recall and precision than \textit{Select-All}. On the other hand, \textit{Select-Cluster} has a much higher recall and a comparable precision with \textit{Select-Best}. Our \textit{Select-Cluster} method achieves the highest F1 score.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/view-spec-q1.png}
  \caption{view specification result on Open data}
  \label{fig:q1}
 \end{figure}

\subsubsection*{\textbf{Q2: Does the view spec stage save user efforts?}} 

In \textit{Select-Cluster}, we first cluster similar columns, then select clusters with the highest score. User interaction can be integrated into $Select-Cluster$ naturally. Instead of let DoD choose clusters based on cluster score,  we could show clusters to users and let them make the decision. In this section, we will look into if user interaction is introduced to view specification, how much user efforts will be needed. To estimate user efforts, we come up with the following two metrics.
\begin{myitemize}
    \item \textbf{Number of clusters} The less the number of clusters is, the less user effort is needed. 
    \item \textbf{Purity of each cluster} The purity of one cluster measures how well one cluster contains a single class (relevant or irrelevant). If most clusters have high purity scores, DoD can show users a random candidate inside one cluster instead of showing the entire cluster, which further reduces user effort.
\end{myitemize}

\autoref{fig:q2} shows the relation between the number of columns and the number of clusters. Generally speaking, the number of clusters increases as the number of candidate columns increases. However, the number of clusters remains relatively low compared to the number of columns. This suggests that if we involve user interaction in the view specification stage, users will only need to go through a small number of clusters.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{figures/view-spec-q2.png}
  \caption{the number of columns and the number of clusters}
  \label{fig:q2}
 \end{figure}

\autoref{fig:purity} shows most clusters have a high purity score. More than 76\% of the clusters have purity scores large than 0.8 and more than 71\% of the clusters have purity scores large than 0.9.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{figures/view-spec-purity.png}
  \caption{Histogram: purity scores of clusters}
  \label{fig:purity}
 \end{figure}

==> tables/new-sota-table.tex <==
\begin{table}[ht!]
\footnotesize
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline 
     & \textbf{Technique}  &  \textbf{Type} & \textbf{\specialcell{Supports \\ Pathless}} & \textbf{\specialcell{Handles\\Example\\Noises}} & \textbf{\specialcell{Output\\Interface}} \\
       \hline\hline
       \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{QBE}}} & MWeaver \cite{mweaver} & S & N & N & Top-k \\
        \cline{2-6}
       & Shen et al. \cite{shen14} & A & N & \specialcell{Fuzzy\\matching} & All\\
       \cline{2-6}
       & FastTopK \cite{s4}& S &  N & \specialcell{Scoring\\model} & \specialcell{Top-k} \\
        \cline{2-6}
        & LearnJoin \cite{bonifati}& A & \specialcell{$Y^1$} & N & \specialcell{Top-1} \\
       \cline{2-6}
        & SQuID \cite{squid} & S & N & N & \specialcell{Top-1}\\
       \cline{2-6}
        & DuoQuest \cite{duoquest} & S & N & \specialcell{Nat. lang.\\queries} & \specialcell{Top-k} \\
        \hline       \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{QRE}}} & TALOS \cite{qbo} & S & N & N & Top-k \\
       \cline{2-6}
        & Sarma et al. \cite{view_definition} & A & N & N & Top-1 \\
        \cline{2-6}
        & SQLSynthe\cite{sql-synthesizer} & S & \specialcell{N} & N & \specialcell{Top-k} \\
        \cline{2-6}
        & Zhang et al. \cite{complex_join_queries} & A & N & N & All\\
       \cline{2-6}
        & Li et al. \cite{hao}& A & N & N & \specialcell{Top-1} \\
       \cline{2-6}
       & PALEO-J \cite{paleo-j} & S & N & N & Top-k\\
       \cline{2-6}
       & SCYTHE \cite{scythe} & A & N & N & \specialcell{Top-k} \\
       \cline{2-6}
       & REGAL \cite{REGAL} & A & N & N & All \\
       \cline{2-6}
        & REGAL+ \cite{regal-plus} & S & N & N & All \\
       \cline{2-6}
       & FastQRE \cite{fastqre} & A & N & N & Top-1 \\
       \hline
       & \textbf{\sys{}} & \textbf{S} & \textbf{Y} & \textbf{Y} & \textbf{\specialcell{signals \& \\  navigation}}\\
       \hline
    \end{tabular}
    \caption{Comparison of prior techniques based on the different challenges addressed. (S = System, A = Algorithm, $Y^1$ = requires Cartesian product on relevant tables)}
    \label{tab:comparison}
\end{table}

% $Y^2$ = supports pathless through joining columns of the same name or type




==> tables/sota-table.tex <==
\begin{table*}[ht!]
\footnotesize
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline 
    Technique  &  Approach & \specialcell{Requires \\ path info} & \specialcell{Dataset \\ Noise} & Scale &  \specialcell{Example \\ Noise} & User feedback \\
       \hline\hline
       Squid \cite{squid} (QBE) & System & Y & N & ? & N & \specialcell{Returns a single \\SQL query (and the \\corresponding output).} \\
       \hline
       Duoquest \cite{duoquest} (QBE)& System & Y & N & & \specialcell{Uses NLQs (natural \\language queries) to \\ alleviate ambiguity \\from user input} & \specialcell{Returns a list of \\top-k SQL queries\\ (and the corresponding output).} \\
       \hline
       S4 \cite{s4} (QBE)& System &  Y & & & \specialcell{use a scoring model \\to handle example noise} & \specialcell{Returns a list of \\top-k SQL queries\\ (and the corresponding output).} \\
       \hline
       \specialcell{Bonifati et al. \cite{bonifati} (QBE?) \\Learning Join queries\\ from user examples \\ \yg{how to classify this} } & \specialcell{help users learn join predicate through user \\tuples and let users label positive \\or negative. Note users are not providing \\ examples, examples are presented to them.\\ this approach needs to know all\\ relevant tables of a join query in advance.\\ The only unknown variable is the join predicate\\ (they do not assume any integrity constraint).}  & N & N & \specialcell{needs to do\\ Cartesian join \\ between \\ relevant tables}& \specialcell{users do not provide \\examples. example tuples \\ are presented to users} & \specialcell{for each tuple presented,\\ the user needs to label\\it as positive or negative} \\
       \hline
       \specialcell{Shen et al. \cite{hao} (QBE) \\ Discovering Queries based \\ on example tuples} & \specialcell{This is the prior work of S4. \\ It assumes a valid query should \\ output a view that contain all the rows in\\ the example table. Its contribution is an\\ algorithm that can fast identify valid\\ queries among all candidate queries.} & Y & N & \specialcell{needs to generate \\ a new database \\ instance in \\ every iteration} & \specialcell{use fuzzy string matching \\ i.e. the constraint is $x \subseteqq y$ \\not $x = y$. Cannot handle \\ other types of noise\\such as domain error \\or relation error} & N\\
       \hline
        \specialcell{MWEAVER \cite{mweaver}(QBE) \\ Sample-Driven Schema Mapping}  & \specialcell{Given a database D and a view V \\ over it, find a query Q that best \\captures the relation between D and V.\\ (trade-off between approximation and\\ succinctness)} & Y & N & ? & \specialcell{No example information \\ is involved. Query output \\ is given.} & N \\
       \hline
       \specialcell{Li et al. \cite{hao} (QRE) \\ Query From Examples\\ an iterative, data-driven \\ approach to query\\ construction} & \specialcell{First, a user needs to provide an \\example database-result pair (D, R). Then\\ the system will generate and present users a\\ sequence of slightly modified (D, R) pairs. The\\ system can identify the target query based on\\ user's feedback to the modified pairs } & Y & N & \specialcell{needs to generate \\ a new database \\ instance in \\ every iteration} & N & \specialcell{for each (D, R) pair, \\ the user needs to label\\ it as positive or negative} \\
       \hline
       \specialcell{PALEO \cite{paleo}(QRE) \\ Exploring Databases via \\ Reverse Engineering Ranking} & \specialcell{reverse engineering topk queries.\\ The input is a list of values, the output\\ is a set of queries that can produce \\ the similar ranking.} & Y & N & ? & N & N \\
       \hline
       \specialcell{Tran et al. \cite{qbo}(QRE) \\ Query By Output (TALOS)}  & \specialcell{Given a output of query Q, construct \\ Q' that has the same output as Q} & Y & N & ? & \specialcell{No example information \\ is involved. Query output \\ is given.} & N \\
       \hline
       \specialcell{Sarma et al. \cite{view_definition}(QRE) \\ Synthesizing view definition \\ from data}  & \specialcell{Given a database D and a view V \\ over it, find a query Q that best \\captures the relation between D and V.\\ (trade-off between approximation and\\ succinctness)} & Y & N & ? & \specialcell{No example information \\ is involved. Query output \\ is given.} & N \\
       \hline
      
    \end{tabular}
    \caption{Comparison of prior techniques based on the different challenges addressed. \sg{To discuss: Should we add characteristics also? Like type of query -- similar to the one in duoquest.} \yg{how should we define "scale"?}}
    \label{tab:old_comparison}
\end{table*}
